Data Flow Analysis of Asynchronous Systems using Infinite Abstract Domains

Asynchronous message-passing systems are employed frequently to implement distributed mechanisms, protocols, and processes. This paper addresses the problem of precise data flow analysis for such systems. To obtain good precision, data flow analysis needs to somehow skip execution paths that read more messages than the number of messages sent so far in the path, as such paths are infeasible at run time. Existing data flow analysis techniques do elide a subset of such infeasible paths, but have the restriction that they admit only finite abstract analysis domains. In this paper we propose a generalization of these approaches to admit infinite abstract analysis domains, as such domains are commonly used in practice to obtain high precision. We have implemented our approach, and have analyzed its performance on a set of 14 benchmarks. On these benchmarks our tool obtains significantly higher precision compared to a baseline approach that does not elide any infeasible paths and to another baseline that elides infeasible paths but admits only finite abstract domains.

==> backward.tex <==
\section{backward}
\label{sec:backward}

==> bdfas-illus.tex <==

\begin{figure}
	\centering
  \begin{tabular}{|l|l|l|c|c|}\hline
    & \parbox{0.7in}{Path from worklist} &
    \parbox{0.9in}{Extended path $p$} &
    \demandp{p} & \ptf{p} \\\hline
    1 & & \vpath{hijk} & 3 & \id   \\
    2 & \vpath{hijk} & \sout{\vpath{(hijk)^2}} & 6 & \id  \\
    3 & \vpath{hijk} & \vpath{qhijk} & 3 & \id   \\ \hline
    4 & \vpath{qhijk} & \multicolumn{3}{|c|}{Invoke \textsc{ComputeEndToEnd}(\texttt{foo}, 3)}    \\ \hline
      & \multicolumn{4}{|c|}{\vdots} \\ 
    5 & \vpath{p(cdefgm)^2co(no)^2qhijk} & \vpath{abp(cdefgm)^2co(no)^2qhijk} & 0 & t'=1,x'=x+2,y'=x+1,z'=1  \\
    6 & \vpath{p(cdefgm)^3co(no)^3qhijk} & \vpath{abp(cdefgm)^3co(no)^3qhijk} & 0 & t'=1,x'=x+3,y'=x+2,z'=1  \\
    7 & \vpath{p(cdefgm)^4co(no)^4qhijk} & \sout{\vpath{abp(cdefgm)^4co(no)^4qhijk}} & 0 & t'=1,x'=x+4,y'=x+3,z'=1 \\\hline
        
  \end{tabular}
  \caption{Illustration of algorithm~\ref{algo:main} on running example}
  \label{fig:intra-illus}
  
    \begin{tabular}{|l|l|c|c|}\hline
  	& \parbox{0.9in}{New path $p$ for $\sIVCPaths{\mathtt{foo}}{3}$} &
  	\demandpd{p}{3} & \ptf{p}  \\ \hline
  	1 & \vpath{co} & 3 & \id   \\
  	2 & \vpath{cdefgmcono} & 2 & t'=z,x'=x+1,y'=x,z'=1  \\
  	3 & \vpath{(cdefgm)^2co(no)^2} & 1 & t'=1,x'=x+2,y'=x+1,z'=1  \\
  	4 & \vpath{(cdefgm)^3co(no)^3} & 0 & t'=1,x'=x+3,y'=x+2,z'=1  \\
  	5 & \vpath{(cdefgm)^4co(no)^4} & 0 & t'=1,x'=x+4,y'=x+3,z'=1  \\
  	6 & \sout{\vpath{(cdefgm)^5co(no)^5}} & 0 & t'=1,x'=x+5,y'=x+4,z'=1    \\\hline
  \end{tabular}
  \caption{Illustration of procedure \textsc{ComputeEndToEnd}  invoked with parameters (\texttt{foo}, 3) }
  \label{fig:inter-illus}
\end{figure}


==> challenges.tex <==
%\section{Challenges in Analyzing Asynchronous Programs}
%\label{sec:challenges}


\subsection{Running example}
\label{ssec:inter:illustrativeExample}

\begin{figure}
	\centering
	\includegraphics[trim = 0 170 0 100, clip, scale=0.35]{challengeFig-emb.pdf}
	\caption{Running Example: A simple message passing system}
	\label{fig:challenge}
\end{figure}

Figure~\ref{fig:challenge} depicts our running example, which is a simple
message passing system, with a single process. There is only one channel
and one type of message in the system, and therefore the queuing vector for
any transition is a vector of size 1. The transitions labeled $\langle+1
\rangle$ represent send operations, while the transitions labeled $\langle
-1 \rangle$ represent receive operations.  The process writes to and reads
from four memory locations, namely, $t,x,y,$ and $z$. The first loop
repeatedly sends the messages. The second loop repeatedly tries to receive
three messages in each iteration. Thus, by the time the variables are
referred to in the second loop, the first loop must have iterated at least
twice (there is a message send before the first loop). After two iterations
of the first loop, the values of both $t$ and $z$ are always equal to
1. Therefore, a data flow analysis should ideally be able to infer these
constant values for $t$ and $z$ at node $k$.

\subsection{Potential solution approaches}
\label{ssec:inter:naivesolutions}

In this part of this section, we first discuss some natural attempts to
solve the problem, but that happen to not work. Then, drawing on the
intuitions from this discussion, we give a high-level overview of our
actual proposed approach.

The first natural idea is based on the forward \emph{coverability}
construction of Karp and Miller~\cite{karp1969parallel}. The idea would be
to visit configurations of the system  by forward traversal. To finitize
the number of configurations that are visited, certain abstractions are
carried out, as mentioned below. 

%% In our example,
%% a configuration would be a tuple consisting of a node of the
%% system, the number of messages in the channel currently, and the values of
%% the four variables. To finitize the traversal, the following actions are
%% taken:

\begin{itemize}
\item Whenever a configuration $t$ reaches a node such that some
  predecessor configuration $s$ of $t$ had previously reached the same
  node, and $t$ has more messages in the channel than $s$ had (assume a
  single type of message for simplicity), the number of messages in the
  channel of this type in $t$ is abstracted to $\omega$, where $\omega$
  intuitively represents an arbitrarily high value. An $\omega$ in a
  configuration remains that way no matter how many receive operations this
  configuration subsequently flows through.

  This is basically Karp and Miller's original suggestion to finitize the
  set of message counts that are enumerated.

\item When two configurations arrive at a node with the same number
  of messages in the channel, \emph{join} the two configurations into a
  single one, with value $\top$ for variables whose values differ in the
  two configurations.

  We are suggesting this \emph{over-approximation} to finitize the variable
  values that are enumerated during the traversal.
\end{itemize}

%% %% We first discuss some potential strategies, which can be used to compute the JOFP solution in a sound and precise manner. We use the system from Figure~\ref{fig:challenge} for illustration. We will use the Constant Propagation(CP) lattice for the data values, with the variable ordering as $\langle $t, x, y, z $\rangle$. 

%% %% The infinite configuration space due to arbitrarily high counters can be handled by
%% %% the over-approximation of configuration space using some suitable closed-form
%% %% expressions. We illustrate a natural extension of one such popular
%% %% algorithm, known as coverability-tree construction~\cite{karp1969parallel},
%% %% for data flow analysis in Figure~\ref{fig:overapproxtrace}. Let the
%% %% algorithm explore the configurations in the system given in
%% %% Figure~\ref{fig:challenge}.

\begin{figure}
	\centering
	\includegraphics[trim = 0 280 0 180, clip, scale=0.42]{overapproxtrace-emb.pdf}
	\caption{Configurations generated by the over-approximation based approach}
	\label{fig:overapproxtrace}
\end{figure}

Figure~\ref{fig:overapproxtrace} depicts one such traversal for our running
example, which generates a sequence of configurations.  The initial
configuration is $(a, 0, \langle 0,0,0,0 \rangle)$. Here, $a$ is the
initial node of the system, 0 is the number of messages in the channel, and
all variables have value 0. The variables are depicted in the order
t,x,y,z. The path then moves to node $b$, then node $c$, and then visits
node $c$ two more times by following two iterations of the cycle $\vpath{c
  d e f g}$. Note, the configuration that reaches $c$ after one iteration
of the cycle has its message count abstracted from 2 to $\omega$ (as
indicated by the strikeout and replacement).

After the second iteration of the first cycle, due to joining of two
configurations both with a message count of $\omega$, all variables (except
z) become $\top$ (i.e., not a constant). This configuration now reaches
node $k$, because $\omega$ is able to go through three receive
operations. This causes variable $t$ to be declared ``not a constant'' at
node $k$. This imprecision occurs due to abstraction of counts to $\omega$
and due to joining of variable values across multiple configurations.

%% The exploration then uses the edges in the transition system of Figure~\ref{fig:challenge} to obtain the next configurations $(b, 0, \langle 0,0,0,0 \rangle)$, and $(c, 1, \langle 0,0,0,0 \rangle)$. Figure~\ref{fig:overapproxtrace} shows the exploration of the first loop (shown using single dotted edge), after which we get the state $(c, 2, \langle 0,1,0,1 \rangle)$. As the newly obtained state has an ancestor in the exploration trace with lower number of pending messages (i.e., 1) for the same node, we over-approximate the number of pending messages in this state using a special symbol $\omega$. $\omega$ represents arbitrarily high value of pending messages, thus, the receive operations never block at $\omega$, and the number of pending messages remains $\omega$ hereafter. The exploration continues, and obtains another state $(c, \omega, \langle 1,2,1,1 \rangle)$ (shown in the trace as a struck-out value). As there are two states with node $c$ and pending messages $\omega$, we perform the second kind of abstraction, and join the variable values of the states with nodes $c$ and pending messages $\omega$. Hence, the next state in trace is $(c, \omega, \langle \top, \top, \top, 1 \rangle)$. The exploration continues with this state, and eventually obtains the state $(k, \omega, \langle \top, \top, \top, 1 \rangle)$. The final state signifies that the variable t is not a constant at $k$.

%% As discussed previously, t is a constant at $k$. Hence this approach is imprecise. This imprecision results due to the eager acceleration at state $(c, 2, \langle 0,1,0,1 \rangle)$ . The algorithm ends up including the infeasible path that iterates the first loop once, and then iterates the second loop once. But eager acceleration and joining is essential for the algorithm termination. Therefore, over-approximation may not be the most promising direction.

A different solution strategy would be to design an approach based on
\emph{under-approximation}. The idea would be to enumerate paths of configurations
of the system, employ no abstraction of counts or joining of values in
configurations. Termination could be achieved by throwing away a path if
the join of values brought by previously enumerated paths reaching the same
node dominates the values brought by this path.

By this approach, in the running example, considering node $c$, the
following three paths that end at this node would first be enumerated:
$p_1= \vpath{a b c}$, $p_2 = \vpath{a b c d e f g c}$, and $p_3 = \vpath{a
  b (c d e f g)^2 c}$. The configurations at $c$ due to these paths would
be $(1, \langle 0,0,0,0 \rangle), (2, \langle 0,1,0,1 \rangle),$ and $(3,
\langle 1,2,1,1 \rangle)$, respectively. The join of the variable values
due to these configurations happens to be be $\langle \top, \top, \top, 1
\rangle$.  The next path to be enumerated would be $p_4 =
\vpath{ab(cdefg)^3c}$, which brings the configuration $(4, \langle 1,3,2,1
\rangle)$. As the variable values due to $p_4$ are dominated by the join of
the values due to the previous paths reaching the same node, we drop
$p_4$. Subsequently, the so-far generated paths, namely, $p_1,p_2,$ and
$p_3$, are attempted to be extended to node $k$. Only one of these paths,
namely, $p_3$, has placed enough messages into the channel to be able to go
past three receive operations and reach node $k$.  Therefore, the algorithm
generates just a single path that extends to $k$, i.e.,
$\vpath{ab(cdefg)^2chijk}$. Due to this, the algorithm would conclude that
the values of the variables at node $k$ can only have the values brought by
this path, which are t=1,x=2,y=1,z=1. In other words, all four variables
would be declared as constants.

However, this is clearly unsound. If the path $p_4$ had also been
enumerated, it would have brought values t=1,x=3,y=2,z=1 at node $k$, thus
leading to only t and z being declared as constants. This is the sound
result. The problem is that the minimum number of iterations of each cycle
that need to be taken to obtain a sound result is sensitive to the
statements along the cycle. This upper bound could be arbitrarily high, and
it is not easy to see how to determine this upper bound apriori. 



%% Due to the presence of only a single path being extensible to $k$, the algorithm concludes that the values of variables x and y are constants at $k$. This is clearly an under-approximation as due to another path $\vpath{ab(cdefg)^3chijk}$, the values of x and y at $k$ are 3 and 2 respectively. Hence, they are not constants. The termination condition in the algorithm did not completely reflect the fact that more extensions are required at $c$ in order to get sufficient paths at $k$. Also, it is not always possible to provide a generic bound on the number of extensions required for soundness, as the number is highly sensitive to the structure of the system graph, and can become arbitrarily high. For example, in Figure~\ref{fig:challenge}, the number of receive operations can be increased to any arbitrary number, thus increasing the extensions required.

%% As evident, simple strategies are not sufficient for computing the JOFP in a sound and precise manner. 


==> dfas-macros.tex <==
\newcommand{\ptf}[1]{\ensuremath{\mathit{ptf}({#1})}} %path transfer function
\newcommand{\demandp}[1]{\ensuremath{\mathit{demand}({#1})}} %demand
\newcommand{\demandpd}[2]{\ensuremath{\mathit{demand}({#1}, {#2})}} %demand
\newcommand{\id}{\ensuremath{\mathit{id}}} % identity transfer function
\newcommand{\join}{\ensuremath{\sqcup}}
\newcommand{\bigjoin}{\ensuremath{\bigsqcup}}
\newcommand{\dlattice}{\ensuremath{\mathcal L}}
\newcommand{\flattice}{\ensuremath{\dlattice \rightarrow \dlattice}}
\newcommand{\dominates}{\ensuremath{\sqsupseteq}}

\newcommand{\nodes}{\ensuremath{\mathit{Nodes}}}
\newcommand{\edges}{\ensuremath{\mathit{Edges}}}
\newcommand{\send}[2]{\ensuremath{\mathrm{#1}\,!\,\mathrm{#2}}}
\newcommand{\recv}[2]{\ensuremath{\mathrm{#1}\,?\,\mathrm{#2}}}

\newcommand{\sPathsName}{\ensuremath{\textit{sPaths}}}
\newcommand{\sPaths}[1]{\ensuremath{\sPathsName({#1}})}
\newcommand{\worklist}{\ensuremath{\mathit{workList}}}
\newcommand{\coveredName}{\ensuremath{\mathit{covered}}}
\newcommand{\startnode}{\ensuremath{\mathit{start}}}
\newcommand{\targetnode}{\ensuremath{\mathit{target}}}
\newcommand{\fls}{\ensuremath{\mathit{false}}}
\newcommand{\tru}{\ensuremath{\mathit{true}}}
\newcommand{\concat}{\ensuremath{.}}
\newcommand{\zerovector}{\ensuremath{\overline{0}}}
\newcommand{\cover}[1]{\ensuremath{\mathit{Cover(#1)}}}

\newcommand{\vpath}[1]{\ensuremath{\mathit{#1}}}

% Kumar's macros
\newcommand{\ol}[1]{\ensuremath{\overline{#1}}}
\newcommand{\Path}[1]{\ensuremath{\stackrel{#1}{\longrightarrow}}}
\newcommand{\Move}[1]{\ensuremath{\stackrel{#1}{\rightarrow}}}
\newcommand{\below}{\ensuremath{\leq}}
\newcommand{\latbel}{\ensuremath{\sqsubseteq}}
\newcommand{\latabv}{\ensuremath{\sqsupseteq}}
\newcommand{\dist}{\ensuremath{dist}}
\newcommand{\length}{\ensuremath{\ell}}
\newcommand{\elength}{\ensuremath{e\mathbb{\ell}}}
\newcommand{\lbound}{\ensuremath{\mathbf{L}}}
\newcommand{\jop}{\ensuremath{\mathrm{JOP}}}
\newcommand{\Cov}{\ensuremath{\mathrm{Cov}}}
\newcommand{\compComp}{\ensuremath{\mathbf{A}}}
\newcommand{\compJoin}{\ensuremath{\mathrm{B}}}
\newcommand{\compCompare}{\ensuremath{\mathrm{C}}}
%\newenvironment{proof}{\noindent{\bf Proof:}}{\qed\medskip}

\newcommand\discuss[1]{\textcolor{blue}{#1}}


%\newcommand{\astatetrans}[1]{\Rightarrow_{#1}}
\newcommand{\astatetrans}{\Rightarrow}
\newcommand{\vcfgtrans}[2]{\xrightarrow{#1,#2}}
\newcommand{\vstatetrans}{\Rightarrow}
\newcommand{\natzero}{\mathbb{N}}

%commands for formal symbols
\newcommand{\process}{\ensuremath{\mathcal{P}}}
\newcommand{\astate}{\ensuremath{\mathfrak{s}}}
\newcommand{\asystem}{\ensuremath{\mathcal{S}}}
\newcommand{\vass}{\ensuremath{\mathcal{W}}}
\newcommand{\vcfggraph}{\ensuremath{\mathcal{G}}}


\newcommand{\counterIndex}[2]{\ensuremath{\textit{counterIndex}\:(#1,#2)}}
\newcommand{\callsite}[1]{\ensuremath{\textit{call-sites}\:(#1)}}


\newcommand{\entrynode}[1]{\ensuremath{\textit{en}_{#1}}}
\newcommand{\exitnode}[1]{\ensuremath{\textit{ex}_{#1}}}
\newcommand{\main}{\texttt{main }}

\newcommand{\sIVCPathsName}{\ensuremath{\textit{sIVCPaths}}}
\newcommand{\sIVCPaths}[2]{\ensuremath{\sIVCPathsName({#1},{#2})}}
\newcommand{\funcs}{\ensuremath{\mathit{Funcs}}}

\newcommand{\stmtno}[1]{\ensuremath{\hspace{15pt} - \hspace{3pt} (#1)}}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

\newtheorem{definition}{Definition}


==> dfasOutline.tex <==
\section{Data Flow Analysis and Asynchronous Systems}
\label{sec:outline}

%dataflow analysis details
%What is it-short

%specify input output- lattice (element, order,join), transfer functions, paths, path transfer function, JOP, JOP equation

Data flow analysis, given a system, attempts to infer the properties of all
possible concrete states that arise during executions using suitable
abstractions. It takes a control flow graph (CFG) of the system as input, and
uses a lattice $\dlattice$ to express important properties of sets of concrete states. Given an initial value $l_0 \in \dlattice$, the analysis computes a \emph{data flow fact} $l \in \dlattice$ for each node $v$ in the CFG, which is a conservative over-approximation of all possible concrete states at $v$ due to all possible runs of the system represented by the given CFG. In data flow analysis, each edge in the CFG is associated with an $\dlattice \rightarrow \dlattice$ \emph{transfer function}. We define the composition $\circ$ of two transfer functions $f_1, f_2 \in (\dlattice \rightarrow \dlattice)$, and $l \in \dlattice$ as $(f_1 \circ f_2)(l) = f_2(f_1(l))$. Each path $p= \vpath{e_1e_2 \ldots e_k}$ in the CFG is associated with a \emph{path transfer function}, represented as $\ptf{p}$, which is given by $f_{e_1} \circ f_{e_2} \ldots \circ f_{e_k}$, where $f_e$ is the transfer function associated with edge $e$.


In data flow analysis, the initial lattice value $l_0$ is propagated along the paths in the CFG, and the analysis tries to compute the join-over-all-paths (JOP) solution for each node in the CFG.  Let $v_0$ be the initial node in the CFG, $l_0$ be the initial lattice value, and $v$ be a target node in the CFG, then the JOP solution at $v$ is given by

$$\mathrm{JOP}(v)= \underset{\textit{p is a path from } v_0 \textit{ to v}}{\bigsqcup} \ptf{p}(l_0) $$


%Soundness and meaning of df analysis - Galois connection, concrete states, over-approximation of concrete states, abstract transfer functions, use in proving the absence of a bug

The soundness of data flow analysis is subject to certain conditions. Let $\mathcal{C}$ be the power set of all possible valuations of program variables and $\dlattice$ be the given lattice, then $\mathcal{C}$ and $\dlattice$ must be related using a pair of functions that form a Galois Connection~\cite{cousot1977abstract} -- the abstraction function $\alpha : \mathcal{C} \rightarrow \dlattice$ and the concretization function $\gamma: \dlattice \rightarrow \mathcal{C}$. For the correctness of the analysis, it is required that if the program runs with $c_0 \in \mathcal{C}$ as the initial concrete variable values, then the analysis should run with a value $d_0 \in \dlattice$ such that $\gamma(d_0) \dominates c_0$. Additionally,  a transfer function $f_{\dlattice} \in \dlattice \rightarrow \dlattice$ should be an abstraction of the corresponding concrete transfer function $f_{\mathcal{C}} \in \mathcal{C} \rightarrow \mathcal{C}$, that is for any $l \in \dlattice$, $\gamma(f_{\dlattice}(l)) \dominates f_{\mathcal{C}}(\gamma(l))$.


%algorithm for jop kildall - conditions, over-approx, distributive, precise. termination condition, widening-narrowing.

Kildall's algorithm~\cite{kildall1973unified} is a fix-point based algorithm that is used to compute an over-approximation of the JOP solution of a program for monotone path transfer functions. Kildall's algorithm computes the precise JOP solution if the path transfer functions are distributive.  For termination, Kildall's algorithm requires the lattice to have finite ascending chains. In order to handle lattices with infinite ascending chains, a technique known as widening is used in conjunction with narrowing~\cite{cousot1977abstract}.

%DF for VCGFS
%introduce running example

\subsection{Running Example}
\label{ssec:running-example}


\begin{figure}
	\centering
	\includegraphics[trim = 0 170 0 100, clip, scale=0.35]{challengeFig-emb.pdf}
	\caption{Running Example: A simple message passing system}
	\label{fig:challenge}
\end{figure}


Before we discuss data flow analysis in the context of asynchronous systems, we will first present the running example. Figure~\ref{fig:challenge} depicts our running example, which is a simple message passing system, with a single process. There is only one channel and one type of message in the system, and therefore the queuing vector for
any transition is a vector of size 1. The transitions labeled $\langle+1
\rangle$ represent send operations, while the transitions labeled $\langle
-1 \rangle$ represent receive operations.  The process writes to and reads
from four memory locations, namely, $t,x,y,$ and $z$. The first loop
repeatedly sends the messages. The second loop repeatedly tries to receive
three messages in each iteration. Thus, by the time the variables are
referred to in the second loop, the first loop must have iterated at least
twice (there is a message send before the first loop). After two iterations
of the first loop, the values of both $t$ and $z$ are always equal to
1. 

It is desirable that a data flow analysis for such a system should ideally be able to infer these constant values for $t$ and $z$ at node $k$. We propose data flow analysis approaches for asynchronous systems in this work. But first we discuss the meaning of data flow analysis for asynchronous systems and present the problem statement.


\subsection{Data Flow Analysis of Asynchronous Systems}
\label{ssec:outline:dfas}

%How VCFG can be viewed as a CFG, associate transfer functions instead of actions. show in example?

Data flow analysis takes as input a control flow graph. The VCFG is essentially a control flow graph, in which the edges are
associated with an action and a queuing vector.  For the data flow analysis
of a given VCFG, we can modify the VCFG as follows -- for each edge $v_1 \vcfgtrans{a}{w} v_2$ in the VCFG, the modified VCFG will have an
edge $v_1 \vcfgtrans{f}{w} v_2$, where $f: \dlattice \rightarrow \dlattice$ is
a transfer function that conservatively
over-approximates the behavior of the concrete action $a$. This is similar to introducing abstract transfer functions in the CFG of the system. For instance, let 
the well-known \emph{Constant Propagation} (CP) abstract domain be our choice of  lattice for illustration. An element of the CP lattice is a mapping of each variable to an integer constant, \emph{or} a special symbol $\top$ representing a non-constant value. A special symbol $\bot \in CP$ represents unreachable value. Given an incoming cp value $C$, the transfer function $f$ for the edge $a \vcfgtrans{f}{w} b$ in our example, can be given as,

$$f(C) = \begin{cases} \bot \hspace{110pt} \mathit{if} \hspace{3pt} C = \bot \\ \lbrace (t,0),(x,0),(y,0),(z,0) \rbrace \hspace{13pt}\mathit{else}\end{cases} $$



and, $w$ is $\langle 0 \rangle$. Similar to CFGs, paths are also associated with transfer functions using function composition in VCFGs.

%talk about feasibility of paths in VCFG, show an infeasible path and point therefore JOP is not enough, define JOFP for VCFG

Paths and their feasibility in this modified VCFG are defined in the same
manner as they were defined in Section~\ref{ssec:vcfg} for VCFGs. For instance, in Figure~\ref{fig:challenge}, the path \vpath{abchij} is an infeasible path. Data flow analysis computes the join-over-all-paths (JOP) solution in general for a given CFG. As in case of VCFGs, paths may be infeasible, we want to compute a more precise \emph{join-over-all-feasible-paths }(JOFP) solution for a VCFG. 


\paragraph{Problem Statement :} Given a lattice $\dlattice$, VCFG with entry node $\startnode$, an ``entry''
lattice value $l_0 \in \dlattice$ at $\startnode$, and a target node $\targetnode$, the
JOFP from {\startnode} to {\targetnode} is defined as follows:

$$ \underset{\substack{p \mbox{ is a feasible path from
			$\startnode$ to $\targetnode$}}}{\bigsqcup} (\ptf{p})(l_0) $$

In this work, we propose approaches to compute the precise or a conservative over-approximation of the JOFP . We present next an overview of the approaches presented in the paper.


\subsection{JOFP Computation and Kildall's Algorithm}
\label{ssec:outline:forward}

%Computation of JOFP - propose the map lattice (def, ordering, join), demo a transfer function, show non-termination in the example.
The first approach utilizes the existing data flow analysis techniques, and extends them to the domain of asynchronous systems.

As discussed previously, Kildall's algorithm is employed to compute an over-approximation of the JOP. In order to compute the JOFP solution for a VCFG using Kildall's algorithm, we need to provide a richer abstract domain. We propose an \emph{elevated} lattice $\dlattice_r$ that maps the VCFG queue configuration (counts of instances of each message) to a lattice value. Let $r$ be the dimension of the given VCFG and $\dlattice$ be the given abstract domain, then $\dlattice_r : \mathbb{N}^r \rightarrow \dlattice$ is the elevated lattice, where the ordering and join is point-wise based on the ordering and join of the underlying lattice $\dlattice$. For instance, in Figure~\ref{fig:challenge}, the transfer function $f : \dlattice_r \rightarrow \dlattice_r$ for the edge  $a \vcfgtrans{f}{w} b$, dimension $r = 1$, and input value $l \in \dlattice_r$ can now be given as,

$$f(l) = \lambda n \in \mathbb{N}. ( \begin{cases}\bot \hspace{110pt} \mathit{if} \hspace{3pt} l(n) = \bot \\ \lbrace (t,0),(x,0),(y,0),(z,0) \rbrace \hspace{13pt}\mathit{else} \end{cases})$$ 

A more interesting transfer function will be of edge $c \vcfgtrans{f_1}{w_1} d$, which can be given as,

$$f_1(l) = \lambda n \in \mathbb{N}. ( \begin{cases}\bot \hspace{110pt} \mathit{if} \hspace{3pt} n = 0 \\ l(n-1) \rbrace \hspace{80pt}\mathit{else} \end{cases})$$ 

Here $w_1$ is $\langle 1\rangle$. Another noteworthy transfer function will be of edge $h \vcfgtrans{f_2}{w_2} i$, given as follows,

$$f_2(l) = \lambda n \in \mathbb{N}. ( l(n+1))$$ 


where $w_2 = \langle -1 \rangle$. 

We can formally argue that the lattice $\dlattice_r$ precisely maps the data flow values to the queue configurations, and does not allow any infeasible paths to be admitted in the JOFP computation. But, as is evident, the lattice $\dlattice_r$ has infinite ascending chains, and therefore Kildall's algorithm may not terminate on it. As mentioned earlier, widening is used to handle such cases, but a widening operator is not available for the domain $\dlattice_r$ in the literature. Thus, we propose another abstraction over this domain to handle the same.

%mention that it is an infinte lattice and hence in general widening will be employed for it, but such an operation is not available yet. Thus, for termination we propose an abstraction - that message count does not change if reached k. show the corresponding transfer function? Discuss the tunable cost and precision.


In order to ensure the termination of Kildall's algorithm, we introduce another lattice $\dlattice_{r,k} : D_{r,k} \rightarrow \dlattice$, where $k \in \mathbb{N}$ and $D_{r,k} = \langle 1..k \rangle^r$, that is each element in $\dlattice_{r,k}$ is a finite map. The ordering and join are still defined in a point-wise manner. The transfer functions are also modified accordingly. For instance, in Figure~\ref{fig:challenge}, the transfer function $f : \dlattice_{r,k} \rightarrow \dlattice_{r,k}$ for the edge $a \vcfgtrans{f}{w} b$, dimension $r = 1$, $D_{1,k} = [ 1..k] $, and input value $l \in \dlattice_{r,k}$ can now be given as,

$$f(l) = \lambda n \in D_{1,k}. ( \begin{cases}\bot \hspace{110pt} \mathit{if} \hspace{3pt} l(n) = \bot \\ \lbrace (t,0),(x,0),(y,0),(z,0) \rbrace \hspace{13pt}\mathit{else} \end{cases})$$ 

The transfer function for the send operation on edge $c \vcfgtrans{f_1}{w_1} d$, will now be given as,

$$f_1(l) = \lambda n \in D_{1,k}. ( \begin{cases}\bot \hspace{110pt} \mathit{if} \hspace{3pt} n = 0 \\ l(n-1) \rbrace \hspace{80pt}\mathit{if \hspace{3pt} n < k} \\ l(k) \join l(k-1) \hspace{60pt} \mathit{if \hspace{3pt} n =k} \end{cases})$$ 

The $\dlattice_{r,k}$ lattice is intended to over-approximate the fix-point solution computed using Kildall's algorithm and the $\dlattice_r$ domain. The send transfer function intuitively means that once a path has at least $k$ instances of a message $M$ pending (i.e., they have not been received), then the analysis can assume that infinite instances of message $M$ have been sent, and hence does not need to maintain concrete counts of the instances of that message. Similar abstractions have been used in previous works as well~\cite{karp1969parallel, jhala2007interprocedural, geeraerts2006expand}. Based on the same intuition, the transfer function of the receive operation of edge $h \vcfgtrans{f_2}{w_2} i$, given as follows,

$$f_2(l) = \lambda n \in D_{1,k}. ( \begin{cases} l(n+1) \hspace{50pt} \mathit{if \hspace{3pt n} < (k-1)} \\ \bot \hspace{73pt} \mathit{if} \hspace{3pt} n = k-1 \\ l(k) \hspace{65pt} \mathit{if \hspace{3pt} n} = k\end{cases})$$ 

It is easy to see that Kildall's algorithm terminates on lattice $\dlattice_{r,k}$, if it terminates on the underlying lattice $\dlattice$. We prove that the lattice allows all valid paths, as well as all infeasible paths that have at least $k$ pending send operations. Therefore, this lattice will include a strictly larger set of paths than $\dlattice_r$. For instance, for $k=1$, in Figure~\ref{fig:challenge}, the JOFP computation using $\dlattice_{r,k}$ will include the path \vpath{abchij} in the computation, whereas, the lattice $\dlattice_r$ will not include it. Hence, the fix-point solution computed by the algorithm using $\dlattice_{r,k}$ is in general more imprecise than the fix-point solution computed using the lattice $\dlattice_r$. It can also be observed that for $k_1 < k_2$, the fix-point computation using lattice $\dlattice_{r,k_1}$ will be more imprecise than the fix-point solution computed using $\dlattice_{r,k_2}$. Another observation is that the execution time of the analysis using lattice $\dlattice_{r,k_1}$ will be in general lesser than the execution time of $\dlattice_{r,k_2}$, owing to the sizes of the lattices $\dlattice_{r,k_1}$ and $\dlattice_{r,k_2}$. 

To summarize, we obtain a customizable approach that uses the current data flow frameworks in a seamless manner, and allows a reasonable trade-off between execution cost and precision. We present this approach in detail in the next section.

%discuss how precision is not guaranteed in the above approach, and a more precise approach is needed. Mention that we propose a backward approach that guarantees precision in inter-proc analyses for a class of infinite domains. Emphasize that the class is expressive to handle wide class of properties and includes well known lattices.

\subsection{A More Precise Data Flow Analysis Approach}
\label{ssec:outline:backward}

As discussed in Section~\ref{ssec:outline:forward}, using Kildall's algorithm along with the abstract lattice $\dlattice_{r,k}$ will compute an over-approximation of the precise JOFP. On the other hand, Kildall's algorithm will not terminate when used with the precise lattice $\dlattice_r$. Owing to the soundness guarantees provided by data flow analysis, it is used extensively to prove the absence of bugs in a program. An imprecise analysis can therefore report a bug, when in reality a program is correct. Therefore, it is highly desirable to obtain a precise data flow analysis approach, in order to reduce such false warnings. 

To address the aforementioned issue, we propose a backward data flow analysis approach in Section~\ref{sec:backward}. The approach computes the precise JOFP of a given asynchronous system for a restricted, but expressive class of infinite abstract domains. The approach has a different form than Kildall's algorithm. It is influenced by the coverability problem of well-structured transition systems~\cite{finkel2001well} such as Petri Nets, Vector Addition Systems~\cite{karp1969parallel}, and lossy channels~\cite{abdulla1996verifying}. We present the details in Section~\ref{sec:backward}.



%end with the objective- generalized dataflow analysis of async systems has been surprisingly unattempted (with the exception of JM)and considering the ubiquity of these systems and the importance of data flow analysis we hope to provide a swiss army knife (put it better) framework that can handle a large class of async systems in a sound manner, with reasonable precision.


Asynchronous systems are ubiquitous and essential in today's day and age, and data flow analysis is an important technique for building reliable and robust systems. It is therefore surprising that no generalized data flow analysis techniques exist for these systems. The problem has been largely ignored in the literature, with the exception of the analysis of asynchronous programs using finite, distributive lattices~\cite{jhala2007interprocedural}. With this work we hope to contribute significantly in this area, and provide a data flow analysis framework that can be tailored to suit the precision and cost requirements of a variety of clients.



==> forward-galois.tex <==
\section{Forward DFAS Approach}
\label{sec:forward}
% Current length ~3.5pages, target - 1.5 pages


%% add glue here from revious section to here plus use the reference
In this section we present our first algorithm -- Forward DFAS -- which in
general computes a conservative over-approximation of the JOFP on a given
iVCFG. 



\subsection{Our approach}
Our approach aims to reduce the propagation of facts along infeasible paths
to the extent possible. The core ideas that underpin our approach are:

\begin{itemize}
\item During the fix-point computation, maintain a mapping from \emph{queue
  configurations} (see Section~\ref{ssec:vcfg}) to data flow facts from the
  given abstract domain $\dlattice$, rather than a single joined data flow
  fact, at each VCFG node.

\item The number of queue configurations can be infinite in
  general. Therefore, to ensure termination, we use ``bounded'' queue
  configurations. These are basically vectors of size $r$ (where $r$ is the
  number of counters in the VCFG) such that no entries in the vectors have
  value greater than $\forwthresh$, where $\forwthresh \geq 0$ is a
  user-given parameter to the approach. The intuition is that a value of
  $\forwthresh$ in an entry of a vector actually represents some (unknown)
  value that is greater than or equal to $\forwthresh$. We denote the set
  of bounded queue configurations as $D_{r,\forwthresh}$.

\item If a pair $d \rightarrow v$ is present in the mapping at a node $q_1$
  in the VCFG, where $d$ is a bounded queue configuration and $v \in \dlattice$,
  and there is an edge $q_1 \vcfgtrans{f}{w} q_2$, then $v$ is propagated
  to node $q_2$ iff the queue configuration $d$ contains positive values in
  the counters that are decremented by the queuing vector $w$ of the
  edge. This is the main feature that blocks propagation along infeasible
  paths. Also, upon propagation, a pair $d' \rightarrow f(v)$ is introduced
  into the mapping at node $q_2$, where $d'$ is the result of $d$ updated
  via the queuing vector $w$ of the VCFG edge.
\end{itemize}

Our approach requires that the given abstract domain $\dlattice$ be a
\emph{complete lattice}. $\dlattice$ can be finite or infinite.
$\dlattice$ either needs to be of \emph{finite height}, i.e., not
have any infinite \emph{ascending chains}, or $\dlattice$ needs to have an
associated widening operator
``$\widen_\dlattice$''~\cite{cousot1977abstract}. CP is an example of a
finite-height infinite lattice, whereas the Octagon
domain~\cite{mine2006octagon} is an example of an infinite height lattice
that comes with an widening operator.

Our approach is structured as an instantiation of Kildall's data flow
analysis framework~\cite{kildall1973unified}. This framework needs a given
complete lattice, the elements of which will be propagated around the VCFG as
part of the fix point computation. The complete lattice $D$ that we use for
this purpose is defined as follows:\\[1em]
\hspace*{1cm} $ D \ \equiv \ D_{r,\forwthresh} \rightarrow \dlattice$\\

The ordering on this lattice is as follows: $(d_1 \in D) \sqsubseteq (d_2
\in D)$ iff $\forall c \in D_{r,\forwthresh}.\ d_1(c)
\sqsubseteq_\dlattice d_2(c)$. If a widening operator $\widen_\dlattice$
has been provided for $\dlattice$, we define a widening operator $\widen$
for $D$ as follows: $d_1 \widen d_2 \ \equiv \ \lambda c \in
D_{r,\forwthresh}. \: d_1(c) \, \widen_{\dlattice} \,d_2(c)$.

We now need to define the abstract transfer functions with signature $D
\rightarrow D$ for the VCFG edges, to be used  within the
data flow analysis. As an intermediate step to this end, we define a
ternary relation $\boundedmovei$ as follows. Any triple $(p, q, s) \in \boundedmovei$
iff
$$
\begin{array}{lr}
  \ (0 \leq p \leq \forwthresh) \ \wedge \\
  \ ( (q \geq 0 \wedge p + q \leq \forwthresh \wedge s = p + q)\: \vee
  & \hspace*{2cm} \mathit{(a)}\\ 
  \ \ \: (q \geq 0 \wedge p + q > \forwthresh \wedge s = \forwthresh)\:
  \vee & \hspace*{2cm} \mathit{(b)}\\
  \ \ \: (q < 0 \wedge p = \forwthresh \wedge 0 \leq s \leq \forwthresh
  \wedge \forwthresh - s \leq -1*q) \: \vee& \hspace*{2cm} \mathit{(c)}\\
  \ \ \: (q < 0 \wedge p < \forwthresh \wedge p + q \geq 0 \wedge s = p +
  q)) & \hspace*{2cm} \mathit{(d)}
\end{array}
$$

We now define a relation $\boundedmove$ on vectors. 
A triple of vectors $(c_1, c_2, c_3)$ belongs to 
relation $\boundedmove$ iff all three vectors are of the same size, and for
each index $i$, $(c_1[i], c_2[i], c_3[i]) \in \boundedmovei$.

The intuition behind $\boundedmove$ is as follows.  Let us consider a
VCFG edge $q_1 \vcfgtrans{f:\dlattice \rightarrow \dlattice}{w} q_2$. If
$c_1$ is a bounded queue configuration at node $q_1$, then, $c_1$ upon
propagation via this edge will become a bounded queue configuration $c_2$ at $q_2$
iff $(c_1, w, c_2) \in \boundedmove$. Lines~(\emph{a}) and~(\emph{b}) in
the definition of $\boundedmovei$ correspond to sending a message;
line~(\emph{b}) basically throws away the precise count when the number of
messages in the channel goes above $\forwthresh$. Line~(\emph{c})
corresponds to receiving a message when all we know is that the number of
messages currently in the channel is greater than or equal to
$\forwthresh$; in this case, the number of messages remaining in the
channel after the receive operation (i.e., the value $s$) ranges from a
maximum of $\forwthresh$ to a minimum of $\forwthresh$ minus the number of
messages received in this transition (which is $-1*w[i]$) but not going
below zero.  Line~(\emph{d}) is key for precision when the channel has less
than $\forwthresh$ messages, as it allows a receive operation to proceed
only if the requisite number of messages are present in the channel.

We now define the $D \rightarrow D$ transfer function for the VCFG edge
$q_1 \vcfgtrans{f}{w} q_2$ as follows:
$$ \fun(l \in D) \ \equiv \ \lambda c_2 \in D_{r,\forwthresh}. \,
   \left(\bigsqcup_{c_1 \mathrm{\ such\ that\ } (c_1,w,c_2) \in \boundedmove}
f(l(c_1))\right) $$

Intuitively, the function above obtains the data fact to be associated with
any bounded queue configuration $c_2$ at node $q_2$, by taking the data
facts associated with all bounded queue configurations $c_1$ at $q_1$ such
that $c_1$ can propagate along the VCFG edge and get transformed to $c_2$,
then applying the given transfer function $f$ to all these facts, and then
joining the results of these applications. 

Given a map $m$ from any domain to $\dlattice$, let $\joinmap(m)$
denote the expression $\sqcup_{c \in \mathit{domain}(m)} m(c)$.  
Let $l_0$ denote following function: $\lambda c \in D_{r,\forwthresh}. \,
\mbox{if $c$ is $\vec{0}$ then $d_0$ else $\bot$}$.

We now invoke Kildall's algorithm using the $\fun$ transfer functions
defined above at all VCFG edges, using $l_0$ as the fact at the ``entry''
to the ``main'' procedure.
After Kildall's algorithm has finished computing the fix point solution, if
$l^D_v \in D$ is the fix point solution at any node $v$, we return the
value $\joinmap(l^D_v)$ as the final result at $v$.

The formulation above extends naturally to inter-procedural VCFGs using
generic inter-procedural frameworks that accommodate arbitrary data flow
lattices,  such as the \emph{call strings}
approach~\cite{sharirPneuliInterproc}. We omit the details of this in the
interest of space. 

\subsection{Illustration}

\begin{figure}
\input{forward-table-short.tex}
\caption{Mappings during data flow fact propagation}
\label{fig:forw-illus}
\end{figure}

Figure~\ref{fig:forw-illus} illustrates a few steps of the propagation of
data flow facts between nodes for the  example in
Figure~\ref{fig:challenge}, assuming
$\forwthresh = 3$. The column headers represent bounded queue
configurations. 

Let us consider the row for node $c$ first. The $\bot$ in the column
labeled $\singlconf{0}$ indicates that there are no paths that reach node
$c$ with  queue configuration $\singlconf{0}$. This is because no path
reaches $c$ without having sent any message, and no path to $c$ contains
any receive edges.  The CP fact in the next column indicates that the
queue configuration $\singlconf{1}$ is mapped to CP fact
$(t = x = y = z = 0)$ at node $c$. This happens due to the path that
does not traverse the first cycle. The next column is due to the path that
traverses the first cycle once. The last column indicates the CP fact due
to the join of CP facts from the set of all paths that traverse the first
cycle two or more times.

The row for node $i$ indicates what happens when the facts in the preceding
row get propagated to node $i$ (from node $c$). The single decrement (i.e.,
receive) operation seen along the way (on the edge $h \rightarrow i$)
basically causes the CP facts associated with configurations $\singlconf{1},
\singlconf{2}$, and $\singlconf{3}$ at node $c$ to get associated with
configurations $\singlconf{0}, \singlconf{1}$, and $\singlconf{2}$,
respectively, at node $i$. Furthermore, the fact associated with the
configuration $\singlconf{3}$ also gets propagated and mapped to the
same configuration at node $i$ (since $\singlconf{3}$ represents 3 or more
messages in the channel). The remaining two rows show the result of
propagation from node $i$ to node $j$, and then from node $j$ to node $k$. 
The rest of the fix point solution computation is omitted from
Figure~\ref{fig:forw-illus} in the interest of brevity.

After the fix point is reached, one can infer the constants at any node by
looking up common constants across the CP facts associated with the
different bounded queue configurations that reach the node (the \emph{join}
operation of the CP domain achieves this).  For instance, at node $j$ the
constant $z = 1$ is inferred, while at node $k$ the constants $t = z = 1$
are inferred. Note that this happens to be equal to the JOFP result (i.e.,
is the most precise result possible) for this example.

The precision of our approach is sensitive to the value of $\forwthresh$.
For instance, for the running example, if
$\forwthresh$ is set to 2 (rather than 3), some more infeasible paths would
be traversed. Only $z = 1$ would be inferred at node $k$, which is a conservative
approximation of the true JOFP. Conversely, the running time of the
approach is inversely proportional to the value of $\forwthresh$.

%% Then, its assumptions and properties. Termination, soundness, and
%% expense. 

\subsection{Properties of our approach}

%% We now give an outline of the argument that our approach computes a
%% conservative approximation of the JOFP. Let $v$ be any VCFG node.
%% We need
%% to prove that the solution computed by our approach (which is an element of
%% the lattice $\dlattice$) dominates the JOFP solution at that node $v$ as
%% per the ordering of the lattice $\dlattice$.
We adopt the correctness proof technique of abstract
interpretation~\cite{cousot1977abstract} to argue the soundness of our
approach.  Let $D_r$ be the set of all vectors of size $r$ of
 natural numbers.  Consider the ``concrete'' lattice $D_c \ \equiv\ D_r
\rightarrow \dlattice$, and the following ``concrete'' transfer function
for the VCFG edge $q_1 \vcfgtrans{f}{w} q_2$: $ \funconc(l \in D_c)
\ \equiv \ \lambda c_2 \in D_r. \, \left(\bigsqcup_{c_1 \in D_r
  \mathrm{\ such\ that\ } c_1 + w = c_2} f(l(c_1))\right)$. Let $j^{D_c}_v
\in D_c$ denote the JOP (join over all paths) solution at $v$ using the
concrete transfer function as defined above at all VCFG edges.  It is easy
to see $\joinmap(j^{D_c}_v)$ is equal to the JOFP solution at $v$ using the
given $\dlattice \rightarrow \dlattice$ transfer functions at all VCFG
edges.  \hfill (A)

%% Let $l^{D}_v$ be the fix point solution at node $v$ computed by our
%% invocation of Kildall's algorithm, and let $j^{D}_v$ denote the JOP
%% solution at node $v$ by using our $\fun$ transfer function at all VCFG
%% edges. It can be shown that $l^{D}_v
%% \sqsupseteq j^{D}_v$~\cite{kam1977monotone}. \hfill (B)

%% TODO: For both j^{D_c}_v and j^D_v, we need to specify the "entry" fact

Let $j^{D}_v$ denote the JOP
solution at node $v$ by using our $\fun$ transfer function at all VCFG
edges.
We define a function $\gamma(l \in D) \ \equiv \ \lambda c \in D_r. \,
l(\mathit{min}(c,\vec{\forwthresh}))$, where $\vec{\forwthresh}$ is a vector of
size $r$ all of whose elements are equal to $\forwthresh$.  In the
appendix that is present in supplementary material for this paper, we
prove that the function $\fun$ is a \emph{consistent
  abstraction} of the function $\funconc$. That is, for any
$d \in D$, $\gamma(\fun(d)) \sqsupseteq \funconc(\gamma(d))$. Given this,
the theorems of abstract interpretation tell us that $\gamma(j^{D}_v)
\sqsupseteq j^{D_c}_v$. From this it can be shown that $\joinmap(j^{D}_v)
\sqsupseteq \joinmap(j^{D_c}_v)$. \hfill (B)

Since our approach is an application of Kildall's algorithm using the
$\fun$ transfer functions, it follows that the result it computes $l^{D}_v$
is such that $l^{D}_v \sqsupseteq j^{D}_v$. Therefore, $\joinmap(l^{D}_v)
\sqsupseteq \joinmap(j^{D}_v)$. This result, in conjunction with
results~(A) and~(B) above, imply that  our approach computes a
conservative over-approximation of the precise JOFP at each node.

%% From the definition of $\gamma$ it follows that $\joinmap(\gamma(j^{D}_v))
%% = \joinmap(j^{D}_v)$. Due to this, and result~(C) above, and due to the
%% monotonicity of the $\joinmap$ function over the ``$\sqsupseteq$''
%% comparison, it follows that $\joinmap(j^{D}_v)) \sqsupseteq
%% \joinmap(j^{D_c}_v)$. From this, and from result~(B) above, it follows that
%% $\joinmap(l^{D}_v)) \sqsupseteq \joinmap(j^{D_c}_v)$. Now,
%% $\joinmap(l^{D}_v))$ is nothing but the output of our approach at node~$v$,
%% while $\joinmap(j^{D_c}_v)$ is equal to the desired JOFP solution at
%% node~$v$ (as per result~(A) above). Therefore, our approach computes a
%% conservative over-approximation of the precise JOFP at each node.

If we restrict our discussion to single-procedure systems, the complexity of
our approach is just the complexity of applying Kildall's algorithm. This
works out to $O(Q^2 \forwthresh^r h)$, where $Q$ is the  number of VCFG
nodes, and $h$ is either the height of the lattice $\dlattice$ or the
 maximum increasing sequence of values from $\dlattice$ that is
obtainable at any point  using the
lattice $\dlattice$ in conjunction with Kildall's algorithm, 
using the given widening operation
$\widen_\dlattice$.
% TODO: if lattice height is finite but not bounded, what to do?

%% We now state the complexity of our approach. We restrict ourselves to
%% single-procedure VCFGs for this discussion.  Let $h$ be the height of the
%% lattice $\dlattice$ in case $\dlattice$ is a finite height lattice, else
%% let $h$ be maximum increasing sequence of values from $\dlattice$ that is
%% obtainable at any point as per the given widening operation
%% $\widen_\dlattice$. Therefore, when we apply Kildall's algorithm using the
%% lattice $D$, the fact maintained at any node can change at most
%% $\forwthresh^r h$ times. Therefore, following the standard complexity
%% computation of Kildall's algorithm, the complexity of our approach works
%% out to $O(N^2 \forwthresh^r h)$.


==> forward-table-short.tex <==
\begin{tabular}{|c|c|c|c|c|}\hline
	Node & \multicolumn{4}{c|}{Mapping} \\\cline{2-5}
	& $\singlconf{0}$ & $\singlconf{1}$ & $\singlconf{2}$ &
	$\singlconf{3}$ \\\hline
	
	$c$ & $\bot$ & $(t = x = y = z = 0)$ &  $(t = y = 0, x = z = 1)$ & 
	$(t = z = 1)$ \\\hline
	
%	$i$ &  $(t = x = y = z = 0)$ &  $(t = y = 0, x = z = 1)$ & 
%	$(t = z = 1)$ & $(t = z = 1)$  \\\hline
	
%	$j$ &  $(t = y = 0, x = z = 1)$ & 
%	$(t = z = 1)$ & $(t = z = 1)$ & $(t = z = 1)$  \\\hline
	
	$k$ & $(t = z = 1)$ & $(t = z = 1)$ & $(t = z = 1)$ & $(t = z = 1)$
	\\\hline
	
\end{tabular}


==> forward-table.tex <==

\begin{figure}
  \begin{tabular}{|l|c|c|c|}\hline
    Node & k = 0 & k = 1 &   k = 3  \\ \hline
    \textit{b} & $0\mapsto \langle 0,0,0,0 \rangle$ & $0\mapsto \langle 0,0,0,0 \rangle$ & $0\mapsto \langle 0,0,0,0 \rangle$    \\ \hline
    \textit{c} & $0\mapsto \langle \top, \top, \top, \top \rangle$  & $1\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle 0,0,0,0 \rangle$, $2 \mapsto \langle 0,1,0,1 \rangle$,  \\ 
     & & & $3\mapsto \langle 1, \top, \top, 1 \rangle$ \\ \hline
    \textit{d} & $0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, \top \rangle$ & $2\mapsto \langle 0,0,0,0 \rangle$, $3 \mapsto \langle \top, \top, \top, 1 \rangle$   \\ \hline
    \textit{e} & $0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, \top \rangle$ &$2\mapsto \langle 0,0,0,0 \rangle$, $3 \mapsto \langle 1, \top, \top, 1 \rangle$     \\ \hline
    \textit{f} & $0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, 1 \rangle$ & $2\mapsto \langle 0,0,0,1 \rangle$, $3 \mapsto \langle 1, \top, \top, 1 \rangle$     \\ \hline
    \textit{g} & $0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, 1 \rangle$ & $2\mapsto \langle 0,0,0,1 \rangle$, $3 \mapsto \langle 1, \top, \top, 1 \rangle$     \\ \hline
    \textit{h} & $0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, \top \rangle$ & $1 \mapsto \langle 0,0,0,0 \rangle$, $2 \mapsto \langle 0, 1, 0, 1 \rangle$      \\ 
     & & & $3\mapsto \langle 1, \top, \top, 1 \rangle$ \\ \hline
    \textit{i} & $0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, \top \rangle$ & $0 \mapsto \langle 0,0,0,0 \rangle$, $1 \mapsto \langle 0, 1, 0, 1 \rangle$      \\ 
     & & & $3\mapsto \langle 1, \top, \top, 1 \rangle$ \\    \hline
  \textit{j} &$0\mapsto \langle \top, \top, \top, \top \rangle$ & $1\mapsto \langle \top, \top, \top, \top \rangle$ & $0 \mapsto \langle 0,1,0,1 \rangle$, $3 \mapsto \langle 1, \top, \top, 1 \rangle$      \\ \hline
    \textbf{\textit{k}} &$\mathbf{0\mapsto \langle \top, \top, \top, \top \rangle}$ & $\mathbf{1\mapsto \langle \top, \top, \top, \top \rangle}$ & $\mathbf{3 \mapsto \langle 1, \top, \top, 1 \rangle}$      \\   \hline
  \end{tabular}
  \caption{Illustration of algorithm on example in
  Figure~\ref{fig:challenge} for 3 different values of k }
  \label{fig:forward-illus}
\end{figure}


==> forward.tex <==
\section{Approximate Data Flow Analysis of Asynchronous Systems using Infinite Abstract Domains}
\label{sec:forward}

%keep the section simple as it is not that complicated anyway. Keep it short and clean. No long winding explanations or ideas.
%main point to convey in this section is the utility  of the simple idea, even if it seems imprecise.
%broad outline
%Assumptions 
%algo description
%algo illustration
%proof outlines
%intrer proc para


%problem statement

Given an abstract data flow lattice $\dlattice$, a VCFG with dimension $r \in \mathbb{N}$, whose ``actions''
are abstract transfer functions from the domain $\flattice$ and whose
starting node is {\startnode}, an ``entry'' data flow value $l_0 \in
\dlattice$ at {\startnode}, and a target node of the VCFG of interest,
denoted as {\targetnode}, our problem is to compute the JOFP from
{\startnode} to {\targetnode} as defined in the previous section. In this section, we propose an approach that conservatively approximates the JOFP. We discuss the interprocedural algorithm at the end of this section.



\subsection{Assumptions}
\label{ssec:forward:assumptions}
%definitions and assumptions
%Kildall restrictions - monotone underlying transfer functions, complete lattice with no infinite ascending chains. In case there are infinite ascending chains then widening operation should be given and associated with suitable edges. 

The approach is based on the same assumptions as Kildall's algorithm. The first requirement is that $\dlattice$ must be a complete lattice with no infinite ascending chains. The $\flattice$ transfer functions must all be monotone. In case the lattice has infinite ascending chains, suitable edges must be associated with transfer functions with widening operators~\cite{cousot1977abstract}. For simplicity, we also assume that each queue operations (send/receive) is associated with an $\mathit{id}$ transfer function. Additionally, we assume for the purpose of presentation that an edge can only send/receive a single message. 

We introduce some additional notation for vectors. For a vector $d \in \langle \mathbb{N} \rangle^r$ of dimension $r$ and index $i \in [1..r]$, $d[i]$ denotes the $i^{th}$ component of the vector $d$. For $n \in \mathbb{Z}$, we use the notation $d_i^{n}$ to denote the vector $d[i \mapsto d[i] + n]$, i.e., a vector that is identical to vector $d$ in all components except $i$, where it is incremented by $n$.



\subsection{Algorithm}
\label{ssec:forward:algo}
%algo description
%State that we will use Kildall's algo as blackbox, but give transfer functions for the given lattice L. Assume that transfer function for channel operations is id. Give general transfer functions for any r and k. Mention that in the outline r was one. Explain how to obtain JOFP from solution - join all entries in the map. Give the trasnfer function for widening as well or mention how it accommodates (similar to non queue operation transfer functions). 

The data flow algorithm is straightforward and uses Kildall's algorithm as a black-box. Our key contribution is in formulating conservative transfer functions, which are reasonably precise. 


Besides the VCFG with dimension $r$, domain $\dlattice$, the start node \startnode, the target node \targetnode, and the initial value $l_0$, our algorithm takes a number $k \in \mathbb{N}$ as input, where $k$ decides the precision of the analysis. Let the set $D_{r,k}$ be the set of vectors of the form $ \langle 1 \dots k \rangle^r$ for any $k,r \in \mathbb{N}$. We analyze the VCFG using the elevated lattice $\dlattice_{r,k}$, where each element is a belongs to the set $D_{r,k} \rightarrow \dlattice$. The ordering and join in this lattice is point-wise. 

The algorithm first converts the initial value $l_0 \in \dlattice$ to the corresponding value $l'_0 \in \dlattice_{r,k}$, as follows :


\begin{equation}
\label{eqn:forward:init}
l'_{0} = \lambda d \in D_{r,k}. (\begin{cases} l_0 \hspace{20pt} \mathit{if} d = \zerovector \\ \bot \hspace{20pt} \mathit{else} \end{cases})
\end{equation}



The algorithm then associates $\dlattice_{r,k} \rightarrow \dlattice_{r,k}$ functions to each edge in the VCFG using the underlying $\flattice$ transfer functions. There are 3 kinds of edges in the VCFG - non-queue operations, send operations and receive operations. We present the generalized $\dlattice_{r,k} \rightarrow \dlattice_{r,k}$ transfer functions for each of them.  For the non-queue edge $e$, with associated transfer function $f \in \flattice$, the $\dlattice_{r,k} \rightarrow \dlattice_{r,k}$ transfer function $f_{r,k}$ for $l \in \dlattice_{r,k}$ can be given as,

\begin{equation}
\label{eqn:forward:nonQ}
f_{r,k}(l) = \lambda d \in D_{r,k}. ( f(l(d)))
\end{equation}

It should be noted that the transfer function in Equation~\ref{eqn:forward:nonQ} does not depend on the type of $f$. Therefore, the transfer function $f$ can be replaced by a function that uses widening operator as well. In this manner our algorithm allows general infinite domains to be applied to asynchronous systems.

For the send operation edge that sends a message m on channel c, let the index corresponding to the (message, channel) pair be $i$ in the VCFG. The underlying transfer function for this edge is $\mathit{id}$ by the assumptions. The generalized $\dlattice_{r,k} \rightarrow \dlattice_{r,k}$ transfer function for this edge will be given as follows,

\begin{equation}
\label{eqn:forward:send}
f_{r,k}(l) = \lambda d \in D_{r,k} . \left( \begin{cases}
\bot \hspace{72pt} \mathit{if} d[i] = 0 \\
l(d_i^{-1}) \hspace{55pt} \mathit{if} d[i] < k \\
l(d) \join l(d_i^{-1}) \hspace{30pt} \mathit{if} d[i] = k
\end{cases}\right)
\end{equation}


As mentioned in Section~\ref{ssec:outline:forward}, the analysis will precisely track the paths where no message has more than $k$ instances. Once the number of instances of any message goes above $k$ along a path, the analysis will not increment or decrement the number of instances  of that message anymore, assuming that infinite instances of that message have been sent along the path. This is the approximation introduced by out algorithm. The transfer function for the send operation represents exactly that. From Equation~\ref{eqn:forward:send}, we can see that for the case where $d[i] = k$, the data flow value is not over-written  (as done in other cases), but is accumulated, approximating the values due to paths with higher values of $d[i]$. In Section~\ref{ssec:outline:forward}, we had presented the transfer functions for $r=1$.
%%Come back here

Similar to Equation~\ref{eqn:forward:send}, the transfer function for receive operation that receives the message m from channel c, where $i$ is the index corresponding to the (message,channel) pair, can be  given as,

\begin{equation}
\label{eqn:forward:recv}
f_{r,k}(l) = \lambda d \in D_{r,k} . \left( \begin{cases}
l(d_i^{1}) \hspace{55pt} \mathit{if} d[i] < (k-1) \\
\bot \hspace{66pt} \mathit{if} d[i] = k-1 \\
l(d) \hspace{57pt} \mathit{if} d[i] = k
\end{cases}\right)
\end{equation}

Similar to Equation~\ref{eqn:forward:send}, Equation~\ref{eqn:forward:recv} precisely admits the paths that do not send more than $k$ instances of any messages and approximates all the paths that send more than $k$ instances of any message at least once.


After providing the initial value and the elevated transfer functions, The VCFG is analyzed using Kildall's algorithm. When the algorithm terminates, each node $v$ is mapped to a value $l' \in \dlattice_{r,k}$. Let $l_{r,k} \in \dlattice_{r,k}$ be the fix-point value computed by the algorithm for the node \targetnode. The value $l \in \dlattice$ at the \targetnode\, node, which over-approximates the JOFP at \targetnode\, is obtained as follows :

\begin{equation}
\label{eqn:forward:jofp}
l = \underset{d \in D_{r,k}}{\bigjoin} l_{r,k}(d)
\end{equation}


\subsection{Illustration}
%algo illustration
%Show some transfer functions which are more complicated (non q, send and receive). Show path transfer function of an interesting path (a feasible and infeasible path for different k). Show the final fix-point solutions of k=0, k=1, k=2 for node k. Show the paths that are infeasible in the higher precision and feasible in the lower precision leading to imprecise answers, show their path transfer functions and the value brought in as well. Decide notation for showing the solution. 
\input{forward-table.tex}


We now illustrate the important parts of the algorithm using example in Figure~\ref{fig:challenge}. 

In the example, the dimension $r$ is 1, and the choice of abstract domain is Constant Propagation (CP). The underlying CP transfer functions are well known in the literature, and are straightforward in this example. Hence we will not be specifying them here. Kildall's algorithm is also widely known, and hence we will not be showing the step by step execution of the fix-point algorithm. We use the notation $\langle a,b,c,d \rangle$ to represent the CP fact $\lbrace (t,a), (x,b), (y,c) ,(z,d) \rbrace$, and the notation $n \mapsto \langle a,b,c,d \rangle $, to represent the fact that at configuration $n$ the data flow value is $\langle a,b,c,d \rangle$. 

Table~\ref{fig:forward-illus} shows the fix-point values computed by Kildall's algorithm for k=0, k=1 and k=3. The configurations which map to $\bot$ are not shown. As discussed in Section~\ref{ssec:running-example}, we are interested in determining the constants at node \textit{k}. From Figure~\ref{fig:forward-illus}, the fix-point solution at node \textit{k} for k=3 is $3 \mapsto \langle 1, \top, \top, 1 \rangle$, i.e., variables \textit{t} and \textit{z} are constants and \textit{x} and \textit{y} are non-constants. This is the most precise solution, and higher values of k will not give us any more precision. 

The loss of precision at k=0 and k=1 is due to the lesser number of configurations being maintained by the transfer functions, which results in joining the values due to different configurations. Consider the paths $ p_1 = \vpath{abc}, p_2 = \vpath{abcdefgc}$, and $p_3 = \vpath{ab(cdefg)^2c}$. Given the initial  value $\lbrace 0 \mapsto \langle 0,0,0,0 \rangle \rbrace$, the value at the end of $p_1$ for k=0 is $ \lbrace 0 \mapsto \langle 0,0,0,0 \rangle \rbrace$ . The value at the end of $p_2$ and $p_3$ are $\lbrace 0 \mapsto \langle 0,1,0,1 \rangle \rbrace$ and $\lbrace 0 \mapsto \langle 1,2,1,1 \rangle \rbrace$ respectively. The join of these values is $\lbrace 0 \mapsto \langle \top, \top, \top, \top \rangle \rbrace$. Similarly, the values at the ends of $p_1, p_2,$ and $p_3$ for k=1 are $\lbrace 1 \mapsto \langle 0,0,0,0 \rangle \rbrace$, $\lbrace 1 \mapsto \langle 0,1,0,1 \rangle \rbrace$, and $\lbrace 1 \mapsto \langle 1,2,1,1 \rangle \rbrace$ respectively. As can be seen, increment in the value of k did not translate to an increment in the precision in this case. On the other hand, for k=3, the values at the ends of $p_1, p_2,$ and $p_3$ are $\lbrace 1 \mapsto \langle 0,0,0,0 \rangle \rbrace$, $\lbrace 2 \mapsto \langle 0,1,0,1 \rangle \rbrace$, and $\lbrace 3 \mapsto \langle 1,2,1,1 \rangle \rbrace$ respectively. the join of these values is $\lbrace 1 \mapsto \langle 0,0,0,0 \rangle , 2 \mapsto \langle 0,1,0,1 \rangle ,3 \mapsto \langle 1,2,1,1 \rangle \rbrace$, which results in increased precision, and hence a precise answer eventually. 



\subsection{Properties of the Algorithm}
\label{ssec:forward:proof}

We present the different properties of the proposed algorithm and their proof outlines in this section. The detailed proofs are available in the supplementary material submitted along with the paper.

\textbf{Theorem (Termination).} The algorithm is guaranteed to terminate if
the given underlying domain $\dlattice$ does not have any infinite ascending chains.

\noindent \textbf{Proof outline.} According to the termination proof of Kildall's algorithm~\cite{kildall1973unified}, if the elevated lattice $\dlattice_{r,k}$ for given $r, k \in \mathbb{N}$ does not have any infinite ascending chains, the algorithm will terminate.

We prove the absence of infinite ascending chains in $\dlattice_{r,k}$ using contradiction. The domain $D_{r,k} = \langle  0..k \rangle^r $ is finite. Thus, the elevated lattice $\dlattice_{r,k} : D_{r,k} \rightarrow \dlattice$, is composed of finite maps. Hence, the only way one can have infinite ascending chains in $\dlattice_{r,k}$ is to have an infinite subset $X \subseteq D_{r,k} \rightarrow \dlattice $ such that the elements in $X$ form an ascending chain. That is, for $l_1, l_2, \dots \in X$, $l_1 \sqsubset l_2 \sqsubset \dots$. By the definition of $\dlattice_{r,k}$, this implies that for at least one $d \in D_{r,k}$, $l_1(d) \sqsubset l_2(d) \sqsubset \dots$. This contradicts the assumption that there are no infinite ascending chains in the underlying lattice. Hence, contradiction. $\Box$

\textbf{Theorem (Correctness).} The algorithm computes a conservative over-approximation of the join over all feasible paths that start at \startnode\, node with entry value $l_0 \in \dlattice$ and end at \targetnode.

For the above proof, it is sufficient to prove a slightly stronger result, stated as follows :

\textbf{Lemma (Abstraction).} For any arbitrary path $p$, let $\ptf{p} : \dlattice \rightarrow \dlattice$ be the path transfer function of \vpath{p} using lattice $\dlattice$. Let $f_p : \dlattice_{r,k} \rightarrow \dlattice_{r,k}$ be the path transfer function of \vpath{p}  using lattice $\dlattice_{r,k}$. $f_p$ over-approximates $\ptf{p}$.

\noindent \textbf{Proof outline.} Before we present the proof, we introduce the operator $\downarrow_p : \langle \mathbb{N} \rangle^r \rightarrow D_{r,k}$ for path $p$. Given a configuration $d$ at the end of path $p$, $\downarrow_p d = d_1$, such that for all $i \in [1 \dots r]$ if path $p$ has reached the value $k$ for the $i^{th}$ counter for some prefix $p'$ of \vpath{p}, then $d_1[i] = k$, else $d_1[i] = d[i]$. The $\downarrow_p$ operator relates the concrete configurations to configurations in $D_{r,k}$ along the path \vpath{p}. It can be easily verified that if path \vpath{p} ends at configuration $d$, and if $f_p :\dlattice_{r,k} \rightarrow \dlattice_{r,k}$ is the path transfer function of \vpath{p} using lattice $\dlattice_{r,k}$, then $f_p(d') = \bot $ for all $d' \neq  \downarrow_p d$ and $f_p(\downarrow_p d) \neq \bot$.


Now, for path \vpath{p} that ends in configuration $d$, we need to prove,

\begin{equation}
\label{eqn:sound-lemma}
f_p(l_0')(\downarrow_p d) \dominates \ptf{p}(l_0)
\end{equation}


where $l_0' \in \dlattice_{r,k}$ is obtained using equation~\ref{eqn:forward:init}.

We prove the lemma using induction on the length of $p$ for each kind of transfer function - non-queue operation, send operation, and receive operation. 

\textit{Base Case :} The base case is an empty path, i.e., the value at \startnode. The proof for the base case follows from Equation~\ref{eqn:forward:init}, as $\downarrow_p \zerovector = \zerovector$.

\textit{Inductive case:} For the inductive case we assume that for the prefix \vpath{p'} of \vpath{p} on length $(n-1)$, Equation~\ref{eqn:sound-lemma} holds.  Consider the non-queue operation transfer function (Equation~\ref{eqn:forward:nonQ}) first. It can be seen that if no prefix of $p'$ reached the value $k$ for any counter $i$, $p$ will also not have such a prefix. Also, both \vpath{p} and\vpath{p'} end at the same configuration $d$. From the induction hypothesis, we are given that $\ptf{p'}(l_0) \sqsubseteq f_{p'}(l_0')(\downarrow_{p'} d)$. Now, as $\ptf{p} = f(\ptf{p'})$ and $f_{p} = f'(f_{p'})$, where $f : \dlattice \rightarrow \dlattice$ and $f' : \dlattice_{r,k} \rightarrow \dlattice_{r,k}$ are the transfer functions for the $n^{th}$ edge in \vpath{p}. From the monotonicity of the transfer functions, it is easy to see that Equation~\ref{eqn:sound-lemma} holds in this case.


We now consider the case for operation \recv{c}{m}, where $i \in [1\dots r]$ is the index corresponding to (c,m). According to Equation~\ref{eqn:forward:recv}, the transfer functions are \id\, for the lattice value and only affect the configurations. Also, if the prefix \vpath{p'} of \vpath{p} of length $n-1$ has reached $k$ for counter $i$ at least once, then the same will be true for \vpath{p}. Based on the form of $p'$, we have the following two cases :

\begin{itemize}
\item The first case is when \vpath{p'} has a prefix that has reached the value $k$ for counter $i$. In that case, let $\downarrow_{p'} d' = d_1$, where $p'$ ends at configuration $d'$. From the hypothesis, we know that $f_{p'}(l_0')(d_1) \dominates \ptf{p}(l_0)$. Due to path \vpath{p}, $(\downarrow_p d) [i] = k = d_1[i]$. Therefore from the hypothesis, Equation~\ref{eqn:sound-lemma} holds.

\item  In the case where $p'$ has not reached $k$ for counter $i$ in any prefix, $(\downarrow_{p'} d')[i]= d'[i]$. Also, $d'[i] < k$. The receive operation decrements the value of counter $i$ by 1 in this case according to Equation~\ref{eqn:forward:recv}. Therefore, $(\downarrow_p d)[i] < (k-1)$. From Equation~\ref{eqn:forward:recv}, this implies that $f_p(l_0')(\downarrow_p d) = f_p'(l_0')(\downarrow_p' d')$. Using induction hypothesis, we can infer that Equation~\ref{eqn:sound-lemma} holds in this case as well. 
\end{itemize}

Thus, the receive transfer function in the elevated lattice is an abstraction of the corresponding transfer function in $\dlattice$.


The final case is that of the \send{c}{m} operation, where $i$ is the index corresponding to (c,m). Again based on \vpath{p'} and \vpath{p}, we have three sub-cases to prove under this case. 

\begin{itemize}
\item The first case is when \vpath{p'} (and hence \vpath{p}) has reached $k$ for counter $i$ in some prefix. As a result $(\downarrow_{p'} d') [i]= k = (\downarrow_p d)[i]$. From the hypothesis we are given that $f_{p'}(l_0')(\downarrow_{p'} d') \dominates \ptf{p'}(l_0)$. From Equation~\ref{eqn:forward:send}, this sub-case satisfies the $d[i]=k$, as once the value of a counter reaches $k$, it never decreases in the $\dlattice_{r,k} \rightarrow \dlattice_{r,k}$ transfer functions. Therefore, $f_p(l_0')(d) = f_{p'}(l_0')(d) \join f_{p'}(l_0')(d_i^{-1})$, which dominates $f_p'(l_0')$. Therefore, from the induction hypothesis, Equation~\ref{eqn:sound-lemma} holds for \vpath{p}.

\item The second case is when \vpath{p'} has not reached the value $k$ for counter $i$ in any prefix, and $d'[i] < (k-1)$. This implies $d[i] < k$. Let $\downarrow_{p'} d' = d_1$ In this case $f_p(l_0')(\downarrow_p d) = f_{p'}(l_0')(\downarrow_{p'} d') $. Also, $\ptf{p}(l_0) = \ptf{p'}(l_0)$. Therefore, from the induction hypothesis, Equation~\ref{eqn:sound-lemma} holds for \vpath{p}.

\item The final case is when \vpath{p'} has not reached the value $k$ for any prefix, but $d'[i] = (k-1)$. This implies $d[i] = k$. Also, $(\downarrow_{p'} d')[i] = (k-1)$, $(\downarrow_p d) [i] = k$, and $\downarrow_{p'} d_i^{-1} = \downarrow_{p'} d'$. From Equation~\ref{eqn:forward:send}, in this case $f_p(l_0')(\downarrow_p d) = f_{p'}(l_0')(\downarrow_{p'} d) \join f_{p'}(l_0')(\downarrow_{p'} d_i^{-1})$ which dominates $f_{p'}(l_0')(\downarrow_{p'} d')$.  From the hypothesis, we have $f_{p'}(l_0')(\downarrow_{p'} d') \dominates \ptf{p'}(l_0)$. Hence, Equation~\ref{eqn:sound-lemma} holds in this case.
\end{itemize}



Equation~\ref{eqn:sound-lemma} holds in all cases above. Hence, we can infer that the algorithm computes a sound approximation of the join over all paths. $\Box$

\subsection{Interprocedural Analysis}
\label{ssec:forward:interproc}

The generality of our proposed approach extends to inter-procedural analysis as well. The elevated transfer functions can be used in conjunction with any existing interprocedural approach for infinite domains like call-strings, functional, or iterative~\cite{sharirPneuliInterproc}. The assumptions on the systems will need to include the assumptions of the interprocedural analysis approach of choice. No additional restrictions will be needed.


We have presented a fairly general approach in this section that provides a reasonable trade-off between cost and precision. We empirically evaluate the approach on cost and precision in Section~\ref{sec:impl-and-eval}.












 

==> inter-approach.tex <==
\subsection{Backward DFAS algorithm -- inter-procedural component}
\label{ssec:inter-algo}

In this section we discuss how Backward DFAS  addresses procedure
calls, including recursive calls. Since the approach is not a standard data
flow analysis formulation, we cannot use standard inter-procedural
frameworks like the call-strings approach. Instead, we build full context
sensitivity into the process that extends paths in the backward direction,
which basically ensures that if a path enters the exit node of
a called procedure from a
return-site node $v_r$ in the calling procedure, then the path eventually
comes back from the entry of the called procedure to the call-site node $v_c$
that corresponds to $v_r$ in the calling procedure.

%% \subsection{Inter-procedural VCFG systems}
%% %% 1. Introduce IVCFG, with example, and introduce related basic terminology.


%% Every VCFG $F \in \funcs$ has a designated ``entry'' node, denoted as
%% $\entrynode{F}$, and a designated ``exit'' node, denoted as
%% $\exitnode{F}$. The ``main'' procedure does not have entry or exit nodes,
%% but has the designated $\startnode$ node.

%% % Following two paragraphs can be deleted

%% We assume  that we have a ``main'' procedure, and a set of other
%% procedures denoted as $\funcs$. Each procedure is modeled as a
%% VCFG. Throughout this section, we abuse terminology and use the terms
%% ``procedure'' and ``VCFG'' interchangeably. Every VCFG $F \in \funcs$ has a
%% designated ``entry'' node, denoted as $\entrynode{F}$, and a designated
%% ``exit'' node, denoted as $\exitnode{F}$. The ``main'' procedure does not
%% have entry or exit nodes, but has the designated $\startnode$ node.  All
%% VCFGs can have two other special kinds of nodes, namely, \emph{call-site}
%% nodes and \emph{return-site} nodes. Every call-site node $v_c$ in a VCFG
%% has a ``corresponding'' return-site node $v_r$ in the same VCFG ($v_c$ and
%% $v_r$ correspond to each other).

%% VCFGs have the standard ``intra-procedural'' edges of the form $v
%% \vcfgtrans{f}{w} w$, where $v$ and $w$ are nodes in the same VCFG, $v$ is
%% any node other than call-site node or exit node, and $w$ is any node other
%% than a return-site node or entry node.  The outgoing edge out of any
%% call-site node $v_c$ is called a ``call edge''; it is an inter-procedural
%% edge, whose target is the entry node of some procedure $F \in \funcs$. From
%% the exit node of the same procedure $F$ there is a ``return edge'' to the
%% return-site node $v_r$ corresponding to $v_c$. This pair of call-edge and
%% return-edge is said to correspond with each other. The main procedure is
%% assumed to be not called by any procedure.

\begin{figure}
  \includegraphics[width=4in]{interprocfig-emb.pdf}
  \caption{Example iVCFG}
  \label{fig:inter-example}
\end{figure}

Figure~\ref{fig:inter-example} depicts an iVCFG with two procedures.
 The upper part of the figure, consisting of nodes $a, b, p, q, h, i,
j, k, l$, is the VCFG of the ``main'' procedure. The remaining nodes
constitute the VCFG of the procedure \texttt{foo}. The solid edges are
intra-procedural edges, while dashed edges are inter-procedural
edges. Nodes $p$ and $q$ are a call-site node and a return-site node,
respectively, and correspond with each other. Similarly, nodes $m$ and
$n$. Node $a$ is the $\startnode$ node. This example happens to have the
same essential behavior as the single-procedure system in
Figure~\ref{fig:challenge}; the only thing is, the first cycle in
Figure~\ref{fig:challenge} is replaced by the (tail) recursive procedure
\texttt{foo} in Figure~\ref{fig:inter-example}.

%% \subsection{Assumptions and definitions}

%% %% 3. Mention two assumptions:

%% %%    (a) Join of transfer functions distributes over composition

%% %%    (b) Only sends inside procedures, no receives.

%% %%    Both assumptions above are not onerous compared to literature. 


%% The approach we propose in this section makes two assumptions (on top of
%% the assumptions mentioned in Section~\ref{ssec:intra-algo}). The first
%% assumption is \emph{right distributivity}: for any $f_1, f_2, f \in
%% \dlattice \rightarrow \dlattice$, $(f_1 \sqcup f_2) \circ f = (f_1 \circ f)
%% \sqcup (f_2 \circ f)$. We believe that it should be possible
%% to relax this assumption, but we leave this for future work. (The approach
%% also requires left distributivity of composition over join as well, but
%% this property follows simply from the definitions of function and join.)

%% The next assumption is more fundamental. It is that the procedures in
%% $\funcs$ may send messages, but not have any ``receive'' statements. Only
%% the main procedure is allowed to perform receive actions from channels (it
%% can send as well). Previous approaches that address other sorts of
%% verification problems for asynchronous systems with recursive procedures
%%  mention the same
%% restriction~\cite{sen2006model,ganty2009verifying}.
%% The previous related approach on dataflow analysis of asynchronous
%% programs~\cite{jhala2007interprocedural} also essentially has the
%% same restriction.

%% %% 2. Define IJOFP problem

%% A path in a multi-procedure system can span multiple procedures. A path is
%% said to be \emph{inter-procedurally valid} if during a traversal of this
%% path, if one pushes a symbol representing the call-site node that is just
%% visited onto a stack whenever the path enters a procedure, and pops the top
%% of the stack whenever the path returns from the exit of a procedure to a
%% return-site node, the symbol popped always represents the call-site node
%% that corresponds to the return-site to which the path is returning. A path
%% is said to interprocedurally valid and complete (IVC) if it is
%% interprocedurally valid and the stack maintained during traversal (referred
%% to above) is empty at the end of the path.

%% The definition of a \emph{feasible} path is the same as in the
%% single-procedure setting; this was defined in Section~\ref{ssec:vcfg}.

%% The path
%% transfer function $\ptf{p}$ of an inter-procedural path $p$ is still the
%% composition of the transfer functions of the edges in the path; call edges
%% and return edges are assumed to have {\id} transfer function.

%% Given a node $\targetnode$ in any of the VCFGs, and an
%% ``entry'' value $d_0 \in \dlattice$ at the $\startnode$ node, our problem
%% is to compute the interprocedurally valid JOFP at $\targetnode$:

%% $$
%% \bigjoin_{\parbox{2in}{\centering $p$ is a feasible and\\interprocedurally valid path\\from
%%   ${\startnode}$ to ${\targetnode}$}} (\ptf{p})(d_0)
%% $$



%\subsection{JOFP algorithm}

%% 4. Point to pseudo-code, and mention how it injects into main algorithm.


%% The ``main'' routine of our inter-procedural algorithm is still
%% routine~\textsc{ComputeJOFP} in Algorithm~\ref{algo:intra}, but with a
%% call ``\textsc{InterProcExt}($p$)'' added after and outside the inner loop
%% in lines~\ref{step:intra:inner-loop-begin}-\ref{step:intra:inner-loop-end}
%% (i.e., just before line~\ref{step:intra:until}).



\begin{algorithm}
	\caption{Routines invoked for inter-procedural processing in Backward
      DFAS algorithm}
	\label{algo:interAny-algo}

	\begin{algorithmic}[1]

      \Procedure{InterProcExt}{$p$}
        \State Let $v_1$ be the first node of $p$
		%%paths for caller, node in caller
		\If{$v_1$ is a return-site node, with an incoming return edge from
          a function  $F_1$}\label{step:inter:retbeg}

		\State
        \begin{minipage}[t]{4.7in}
          Let $v_3$ be the call-site node corresponding to $v_1$,
			$e_1$ be the call-site-to-entry edge from $v_3$ to
            $\entrynode{F_1}$, and $r_1$ be the exit-to-return-site edge from
             $\exitnode{F_1}$ to $v_1$. 
        \end{minipage}
        
			\ForAll{$\vpath{p_1} \in \textsc{ComputeEndToEnd}(F_1, \demandp{p}) $}\label{step:inter:end2end}
			  \State $p_2$ = $\vpath{e_1 \concat p_1 \concat r_1 \concat p}$\label{step:inter:growToCS}

		      \If{\textsc{Covered}($\vpath{p_2}$) returns \fls}
			     \State Add $\vpath{p_2}$ to $\sPaths{v_3}$  and to $\worklist$.\label{step:inter:ivcext}					
		      \EndIf				
			\EndFor
		\EndIf\label{step:inter:retend}		
		
		%%from callee to caller, node in callee
		\If{$v_1$  is the entry node of a function $F_1$}\label{step:inter:enbeg}
			\ForAll{$v_3 \in \callsite{F_1}$}
			\State Let $e_1$ be the call edge from $v_3$ to $v_1$.
            $p_2$ = $\vpath{e_1 \concat p}$.
                \If{\textsc{Covered}($\vpath{p_2}$) returns \fls}
			     \State Add $\vpath{p_2}$ to $\sPaths{v_3}$  and to $\worklist$.					
		      \EndIf	
			\EndFor
		\EndIf\label{step:inter:enend}
		
		\EndProcedure
        
	\Procedure{ComputeEndToEnd}{$F$, $d$}
	
	\Comment{\begin{minipage}{4.8in} Returns a set of paths that covers
        each IVC path from $\entrynode{F}$ to  $\exitnode{F}$ 
        that is able to meet a demand of $d$ after returning from $F$.
	\end{minipage}}

	\ForAll{ $F_i \in \funcs$}
	
	\State Place all $0$-depth paths from $F_i$ in
    $\sIVCPaths{\mathit{F_i}}{d}$ \label{step:e2e:init} 
	
	\EndFor
	
	\Repeat\label{step:e2e:repeat}
	\State pathsAdded = \fls
	
	\ForAll{path template $(\vpath{p_1, p_2,  \ldots, p_n})$   in
      any function $F_i \in \funcs$}\label{step:e2e:inlbeg}

    \State \begin{minipage}[t]{4.6in}Let $F_1$ be the procedure called from the call-site at which
    $p_1$ ends, $F_2$ be the procedure called from the call-site at which
    $p_2$ ends, and so on.
    \end{minipage}
    
	\ForAll{$p_1' \in \sIVCPaths{F_1}{d}$, $p_2' \in \sIVCPaths{F_2}{d},
      \ldots$}\label{step:e2e:holecand}
    
    \State \begin{minipage}[t]{4.4in} Let $p' = \vpath{p_1 \concat e_1
        \concat p_1' \concat r_1 \concat p_2 \concat e_2 \concat p_2'
        \concat r_2 \concat \ldots p_n}$, where each $e_i$ is the call-edge
      that leaves the call-site node at which $p_i$ ends and $r_i$ is the
      return edge corresponding to $e_i$.
	\end{minipage}\label{step:e2e:fillhole}
    
	\If{\textsc{CoveredWithDemand}($p', d$) returns \fls}
	\State Add the path $p'$ to $\sIVCPaths{F_i}{d}$.  pathsAdded = \tru. 
	\EndIf	
	\EndFor		\label{step:e2e:endhole}
	
	\EndFor\label{step:e2e:inlend}
	
	\Until{pathsAdded is \fls\label{step:e2e:until}}	
	
	\State \textbf{return} $\sIVCPaths{F}{d}$
	
	\EndProcedure
	
		\Procedure{CoveredWithDemand}{$p, d$}
		
		\Comment{Returns {\tru} iff there exist a set
				of paths in $\sIVCPaths{F}{d}$ that $d$-cover $p$}
		
		\State $C$ = $\{p' \ | \ p' \in \sIVCPaths{F}{d}, \demandpd{p'}{d} \leq
		\demandpd{p}{d} \}$\label{step:covD:C}
		
		\State \textbf{return} {$(\bigjoin_{p' \in C}\ptf{p'}) \dominates \ptf{p}$}
		
		\EndProcedure
		
		
	\end{algorithmic}
\end{algorithm}

The invocation ``\textsc{InterProcExt}($p$)'' in
Line~\ref{step:intra:callInter} of Algorithm~\ref{algo:intra} addresses
the scenario wherein the starting node of the path $p$ that currently needs
to be extended backward is already at a procedure boundary. 
The routine~\textsc{InterProcExt} is shown in
Algorithm~\ref{algo:interAny-algo}. 
%% If
%% the start node of $p$, namely, $v_1$ is not a return-site node or entry
%% node, then backward extensions from $p$ are handled in
%% Lines~\ref{step:intra:inner-loop-begin}-\ref{step:intra:inner-loop-end} in
%% routine~\textsc{ComputeJOFP} itself.

If the starting node of $p$ is a return-site node $v_1$ in a calling
procedure, we invoke a routine~\textsc{ComputeEndToEnd} (in
line~\ref{step:inter:end2end} of Algorithm~\ref{algo:interAny-algo}).
This routine, which we explain later, returns a set of
\emph{interprocedurally valid and complete} (IVC) paths of the called
procedure $F_1$. An IVC
path begins at $\entrynode{F_1}$, which is the entry node of $F_1$, and
ends at $\exitnode{F_1}$, which is the exit node of $F_1$. An IVC path can
itself contain within it IVC paths of procedures called from $F_1$ (hence
the whole IVC path may contain balanced calls and returns within it). The
returned IVC paths are then prepended before $p$, such that the newly
obtained paths begin at the call-site node corresponding to $v_1$
(line~\ref{step:inter:growToCS} in
Algorithm~\ref{algo:interAny-algo}). These paths are added to $\sPathsName$
if they are not covered by other paths (line~\ref{step:inter:ivcext}).

On the other hand, if the starting node of $p$ is the entry node of some
procedure $F_1$, then  this is handled in
lines~\ref{step:inter:enbeg}-\ref{step:inter:enend}. Here, $p$ is extended
simply via the call edge that comes into $v_1$. 

%% Otherwise, if $v_1$ is a return-site node, this situation is handled in
%% Lines~\ref{step:inter:retbeg}-\ref{step:inter:retend} in
%% routine~\textsc{InterProcExt} in Algorithm~\ref{algo:interAny-algo}. Let
%% $F_1$ be the procedure from which control returns to $v_1$. In this
%% scenario, the approach does \emph{not} enter the procedure $F_1$ from which
%% the return happens and does not grow the path step by step within the body
%% of $F_1$ from the exit of $F_1$. Instead, a
%% routine~\textsc{ComputeEndToEnd} is invoked (in
%% line~\ref{step:inter:end2end}), which returns a set of
%% \emph{interprocedurally valid and complete} (IVC) paths of $F_1$ that
%% suffice for the demand created by $p$. We
%% discuss the routine~\textsc{ComputeEndToEnd} subsequently. An IVC
%% path of a function $F_1$ is an IVC path that begins at
%% $\entrynode{F_1}$ and ends at $\exitnode{F_1}$ (such a path can contain
%% within it an IVC path of a procedure called within $F_1$).  For each IVC
%% path $p_1$ returned by~\textsc{ComputeEndToEnd}, $p$ is extended in the
%% backward direction by the prefix $\vpath{e_1 \concat p_1 \concat r_1}$,
%% where $r_1$ is the return edge coming into $v_1$ and $e_1$ is the call-edge
%% corresponding to $r_1$. The thus-extended paths ($p_2$) start at the
%% call-site node $v_3$ corresponding to the return-site node $v_1$ from which
%% we started the extension. In other words, the extension operation enters
%% and leaves the called procedure $F_1$ in a single step, so to say. The
%% paths $p_2$ are stored in $\sPaths{v_3}$ (line~\ref{step:inter:ivcext}) if
%% they are not already covered by other paths in $\sPaths{v_3}$.


\subsection{Routine \textsc{ComputeEndToEnd}}

This routine is the heart of inter-procedural analysis. Given a procedure
$F$ and a demand vector $d$ (of some path that begins at some return-site
node in a caller of $F$), this procedure returns a (finite) set of IVC
paths of $F$ such that every other IVC path of $F$ that contains enough
``send'' operations to meet the demand $d$ (there could be infinite number
of such
IVC paths in general) is covered by the returned set of paths (we call this
notion $d$-covering). 

We assume for simplicity of presentation that there are no cycles in the
procedures in $\funcs$. This assumption can be relaxed without much
difficulty. Also, there is no loss of generality anyway because we allow
recursion. The routine incrementally populates a group of sets, with the
group consisting of a set named $\sIVCPaths{F_1}{d}$ for each procedure
$F_i \in \funcs$.
%     IVC paths of $F_1$ are added to $\sIVCPaths{F_1}{d}$, for each
% $F_1 \in \funcs$, as the routine's execution proceeds.

A \emph{path template} $(\vpath{p_1, p_2, \ldots, p_n)}$ of any procedure
$F_i \in \funcs$ is a sequence of paths in the VCFG of $F_i$ such that: (a) 
 path $p_1$ begins at node $\entrynode{F_i}$ and path $p_n$ ends at
  node $\exitnode{F_i}$, (b) for all $p_i, 1 \leq i < n$, $p_i$ ends at a
  call-site node, and (c) for all $p_i, 1 < i \leq n$, $p_i$ begins at a
  return-site node $v^i_r$, such that $v^i_r$ corresponds to the call-site node
  $v^{i-1}_c$ at which $p_{i-1}$ ends.


%% The \emph{depth} of an IVC path that contains no IVC paths within it is
%% said to be zero. The depth of any other IVC path $p$ is one more than the
%% depth of the deepest IVC path that is directly contained in $p$.
The routine~\textsc{ComputeEndToEnd} first enumerates and saves all
zero-depth paths (see Line~\ref{step:e2e:init} in
Algorithm~\ref{algo:interAny-algo}). These are basically IVC paths that
contain no call-sites within them.  The routine then iteratively takes a
path template at a time, and fills in the ``holes'' between corresponding
(call-site, return-site) pairs of the form $v^{i-1}_c, v^i_r$ in the path
template with IVC paths of the procedure that is called from this pair of
nodes, thus generating a deeper IVC path (see the loop in
lines~\ref{step:e2e:inlbeg}-~\ref{step:e2e:inlend}).
With no loops, there are a fixed number
of path templates of each procedure. 

%% Each set $\sIVCPaths{F_1}{d}$ is initialized with all 0-depth paths of $F_1$
%% (see Line~\ref{step:e2e:init} in Algorithm~\ref{algo:interAny-algo}). These
%% are paths from $\entrynode{F_1}$ to $\exitnode{F_1}$ that do not contain any
%% procedure calls. Because there are no loops, there are a finite number of
%% such paths.

%% For the VCFG of procedure \texttt{foo}
%% in Figure~\ref{fig:inter-example}, there is a single path-template,
%% which happens to be a sequence of two paths: 
%% $(\vpath{c d e f  g  m}, \vpath{n
%%    o})$. Intuitively, a path template is an \emph{incomplete} IVC
%% path, that can be completed to obtain a (normal) IVC path by replacing the
%% ``hole'' between the end of each $p_i$ and the start of $p_{i+1}$ with an
%% IVC path of the procedure that is called from this hole. 

%% The main loop of this routine
%% (Lines~\ref{step:e2e:inlbeg}-\ref{step:e2e:inlend}) iterates all over path
%% templates in all procedures. For each path template of each procedure
%% $F_i$, and for each pair of adjacent paths $p_j, p_{j+1}$ in the path
%% template, the routine \emph{inlines} all possible IVC paths from
%% $\sIVCPaths{F_j}{d}$ into the ``hole'' that is between $p_j$ and $p_{j+1}$, 
%% where $F_j$ is the procedure that is called from this hole (see
%% Lines~\ref{step:e2e:holecand}-\ref{step:e2e:fillhole}).  In other words, a
%% set of IVC paths of procedure $F_i$ is generated using the chosen path
%% template and using already-generated IVC paths of procedures that are
%% called from this path template. In other words, the routine generates
%% deeper and deeper IVC paths, where the depth of an IVC path is the maximum
%% depth of calls see along within the path.

%% The routine stores any IVC path $p'$ of function $F_i$ that it has
%% generated in the set $\sIVCPaths{F_i}{d}$ only if
%% \textsc{CoveredWithDemand}($p',d$) returns false. 
%% The condition checked by
%% routine~\textsc{CoveredWithDemand} is self-evident. If this routine returns
%% true, we say $p'$ is $d$-covered by the subset of paths in
%% $\sIVCPaths{F_i}{d}$ that belong to the set $C$ (computed in
%% Line~\ref{step:covD:C}). 

The routine completes execution when the currently generated and retained IVC paths
cannot be inlined into any path template to yield a new IVC path of the
calling procedure that is not $d$-covered by other IVC paths that are
already generated and retained. It then returns the set of paths in
$\sIVCPaths{F}{d}$, where $F$ and $d$ are the arguments it was invoked
with.

Note that within a single run of the overall algorithm, the
routine~\textsc{ComputeEndToEnd} could possibly get invoked repeatedly with
the same values for the parameters $F$ and $d$. In such cases, it would be
alright  to cache return values (sets of paths) and return them directly. 

\input{inter-table.tex}

Figure~\ref{fig:inter-illus} depicts a run of this
routine with arguments $F$=\texttt{foo} (see
Figure~\ref{fig:inter-example}) and
$d$=3. This invocation is triggered from procedure~\textsc{ComputeJOFP} in
Algorithm~\ref{algo:intra} due to the path $p \equiv \vpath{q h i j
  k}$, which starts at the return-site $q$, and has demand of 3.
\vpath{co} in Row~1 is a path with no calls (i.e., is a base case). Each
subsequent row shows a deeper IVC path of procedure \texttt{foo} obtained by
filling in the hole in the path template $(\vpath{c d e f g m}, \vpath{n
  o})$ with the IVC path shown in the preceding row. The IVC path in Row~6
is not retained since it is 3-covered by the paths in Rows~4 and~5. Hence,
the algorithm terminates after 4 levels of inlining. Notice the analogy
between this and how the algorithm stopped after iterating the first cycle
four times for the example in Figure~\ref{fig:challenge}, as illustrated in
Figure~\ref{fig:intra-illus}. 

%% Recall that the
%% procedure~\texttt{foo} has single path template, namely, $(\vpath{c d e f g
%%   m}, \vpath{n o})$. The second column in each row indicates the IVC path
%% that was generated in a previous step and that is inlined into the ``hole''
%% in the (sole) path template to generate a new IVC in this step. The new IVC
%% path is indicated in the third column. The fourth and fifth columns are
%% self-explanatory.

%% The path $\vpath{c o}$ is a zero-depth path that the routine generates
%% first (Row 1).  This path is inlined into the hole in the path template to
%% produce a depth-1 path (Row 2, path $\vpath{c d e f g m c o n o}$). The
%% depth-1 path is inlined into the path template to produce a depth-2 path
%% (Row 3). This process continues until a depth-5 path is generated (Row
%% 6). This depth-5 path is discarded (i.e., not stored), because it is
%% 3-covered by the paths generated in Rows~4 and~5. At this point the routine
%% terminates, and returns the five IVC paths shown in Column~3, Rows~1-5, in
%% Figure~\ref{fig:inter-illus}.

Recall that the overall algorithm had invoked
routine~\textsc{ComputeEndToEnd} due to the path suffix $\vpath{q h i j
  k}$. Therefore, after the routine returns, path $\vpath{q h i j k}$ is
prepended with each of the five IVC paths returned by the routine (as
depicted in Figure~\ref{fig:inter-illus}). These five paths are subsequently
extended in the backward direction to reach node $\startnode$=$a$.  The
algorithm now terminates.  At the end of all these paths, the values
$t=1,z=1$ hold, and hence these constant values can be inferred at node
$k$.

\subsection{Properties of the algorithm}
\label{ssec:intra-proof}

We provide brief argument sketches here about the key properties of Backward
DFAS.  Detailed proofs are available in the appendix
that is included with supplementary material for this paper.

\emph{Termination.} The argument is by contradiction.
For the algorithm to not terminate, from Higman's
lemma, it follows that an infinite sequence of paths $p_1, p_2, \ldots$,
such that for all $i$, $\demandp{p_i} \leq \demandp{p_{i+1}}$ must be added
to some set $\sPaths{v}$,  or an infinite sequence of paths $p_1, p_2, \ldots$,
such that for all $i$, $\demandpd{p_i}{d} \leq \demandpd{p_{i+1}}{d}$ must be added
to some set $\sIVCPaths{F}{d}$.
Because the algorithm never adds covered paths,
it follows that for all $i$: $ \bigjoin_{1
  \leq k \leq i+1} \ptf{p_k} \ \sqsupset \bigjoin_{1 \leq k \leq i}
\ptf{p_k} $. However, this contradicts the assumption that the lattice of
transfer functions is of finite height.
%% In the inter-procedural setting, it
%% follows from the observation above that  a finite
%% number of invocations to the
%% routine~\textsc{ComputeEndToEnd} will be made. Each invocation is
%% guaranteed to terminate, using a similar argument as in the preceding
%% paragraph.

\emph{Soundness and precision.}
Let $p$ be any arbitrary feasible
path from $\startnode$ to $\targetnode$. It can be
proved using induction on the length of $p$, using Lemma~1
(Section~\ref{ssec:intra-algo}) in the inductive case's argument, that when
the algorithm terminates, $\sPaths{\startnode}$ contains a set of paths
that cover $p$. Therefore, the covering paths bring data values to $\targetnode$ such
that their join dominates $(\ptf{p})(d_0)$.  In the inter-procedural case,
the argument above can be suitably extended.  Hence,
over-approximation (i.e., soundness) is shown.
To show that the algorithm's output is \emph{precisely} equal to the JOFP,
we need to show that the algorithm's output is an under-approximation
of the JOFP as well. This is easy to see, as the output is a join of the
values brought by a set of zero-demand paths (see
Line~\ref{step:intra:return} in Algorithm~\ref{algo:intra}), which are
feasible paths.
%% Therefore, clearly the algorithm's output is an
%% under-approximation of the JOFP at $v$. This, in conjunction with the
%% over-approximation that we argued above, implies that the algorithm's
%% output is \emph{precisely} equal to the JOFP.

\emph{Complexity.} We show the complexity of our approach in the
single-procedure  setting. Our analysis follows along the
lines of the analysis of the backwards algorithm for coverability in
VASS~\cite{bozzelli2011complexity}.  The overall idea, is to use the
technique of Rackoff~\cite{rackoff1978covering} to derive a bound on the
length of the paths that need to be considered. We derive a complexity bound
of $ O(\Delta.h^2.\lbound^{2r+1}.r.log(\lbound))$,  where $\Delta$ is
the total number of transitions in the VCFG,  $Q$ is the number of VCFG
nodes,  $h$ is the height of lattice of $\dlattice \rightarrow \dlattice$
functions, and $\lbound = (Q.(h+1).2)^{(3r)! + 1}$. 



==> inter-table.tex <==

\begin{figure}
  \begin{tabular}{|l|l|c|c|}\hline
    & \parbox{0.9in}{New path $p$ for $\sIVCPaths{\mathtt{foo}}{3}$} &
    \demandpd{p}{3} & \ptf{p}  \\ \hline
    1 & \vpath{co} & 3 & \id   \\
    2 & \vpath{cdefgmcono} & 2 & t'=z,x'=x+1,y'=x,z'=1  \\
    3 & \vpath{(cdefgm)^2co(no)^2} & 1 & t'=1,x'=x+2,y'=x+1,z'=1  \\
    4 & \vpath{(cdefgm)^3co(no)^3} & 0 & t'=1,x'=x+3,y'=x+2,z'=1  \\
    5 & \vpath{(cdefgm)^4co(no)^4} & 0 & t'=1,x'=x+4,y'=x+3,z'=1  \\
    6 & \sout{\vpath{(cdefgm)^5co(no)^5}} & 0 & t'=1,x'=x+5,y'=x+4,z'=1    \\\hline
  \end{tabular}
  \caption{Illustration of algorithm on example in
  Figure~\ref{fig:inter-example} }
  \label{fig:inter-illus}
\end{figure}



==> intra-approach.tex <==
\section{Backward DFAS  approach}
\label{sec:bdfas}

%% 1. Problem statement.

A limitation of the Forward  DFAS approach is its dependence on the
user-given bound $\forwthresh$; if this is too  low, precision would be
sub-optimal, and if it is too high efficiency will suffer (for no extra precision). 
 The Backward DFAS approach that we present
in this section needs no user-given bound, and is guaranteed to compute the
precise JOFP at any node of the iVCFG (even in the presence of recursive
procedures). Intuitively, the idea behind this approach is to enumerate
paths in the iVCFG in increasing order of path-length in the backward
direction starting from the target node of interest, and find limits on the
number of times these paths need to iterate cycles in an on-demand manner.

%% Let us consider our running example in Figure~\ref{fig:challenge}. The
%% location of interest is the node $k$. The \emph{demand} of a path is
%% intuitively the number of ``receive'' operations in the path that do not
%% have 
%% preceding matching ``sends'' in the same path.
%% % Therefore, feasible paths
%% % have a demand of zero, and infeasible paths have positive demand.
%% Let us first consider how many iterations of the second cycle are
%% needed. Paths that iterate the second cycle once or more and reach node $k$
%% are of the form $\vpath{hijk}, \vpath{(hijk)^2},\ldots,\vpath{(hijk)^i}$,
%% and so on. All these paths have the same path transfer function (see
%% Section~\ref{ssec:prelim:dataflow}), namely, the \emph{identity}
%% function. Also, paths $\vpath{(hijk)^2}$ onward have higher demand than
%% path $\vpath{(hijk)}$. Hence, if any path $p_1$ that can be prepended
%% before $\vpath{(hijk)^2}$ to obtain a feasible path, the same prefix can
%% also be prepended before $\vpath{hijk}$ to obtain a feasible path that also
%% brings the same data values to node $k$. Therefore, we can retain the path
%% $\vpath{hijk}$ and drop all paths $\vpath{(hijk)^i}$, $i > 1$.

%% We now shift attention to the first cycle, and see how many iterations of
%% the first cycle we need to prepend in front of the path $\vpath{hijk}$ that
%% was retained above. The demands of the paths $\vpath{chijk}$,
%% $\vpath{c(defgc)^1 hijk}$, \ldots, $\vpath{c(defgc)^5 hijk}$, are 3, 2, 1,
%% 0, 0, and 0, respectively. We note that five or more iterations of the
%% first cycle do not help. They don't reduce the demand any more than 3 and 4
%% iterations; also they all bring constants $t = 1, z = 1$ to node $k$, which
%% is the same as what is brought by the join of paths that iterate the first
%% cycle 3 and 4 times, respectively (this can be determined using path
%% transfer functions, as will be discussed later in this section). Therefore,
%% the algorithm retains only the set of paths $\vpath{c(defgc)^i hijk}$, $0
%% \leq i \leq 4$. The algorithm then can extend these paths back to node $a$,
%% and then stop. The join of the results brought by these end-to-end paths
%% from $a$ to $k$ is guaranteed to be  the  precise JOFP at node $k$.

%% The intuitive presentation above assumed that we would unroll cycles one
%% iteration at a time. The actual algorithm is more general, and does not
%% depend on identifying cycles in the VCFG at all. We present the actual
%% algorithm formally below.



%% Our actual proposal builds on the under-approximation idea mentioned
%% above. To overcome this difficulty mentioned above, our approach grows
%% paths in the \emph{backward} direction rather than in the forward
%% direction. In the example, starting from node $k$, it first grows the path
%% backward to obtain the suffix \vpath{hijk}. This suffix has a \emph{demand}
%% of three; i.e., it goes through three ``receives'' that are not balanced by
%% preceding ``sends'' within the suffix. Knowledge of this demand confers a key
%% advantage; the approach now iteratively prepends longer and longer prefixes
%% that meet this demand.  The first prefix prepended is $p_3$ ($p_1$ and
%% $p_2$ do not meet the demand of the suffix \vpath{hijk}). This results in
%% the path $p_3 \concat \vpath{hijk}$. The next prefix that is prepended is
%% $p_4$, resulting in the path $p_4 \concat \vpath{hijk}$. These two paths
%% agree on the constant values t=1,z=1 at node $k$; importantly, they
%% disagree on the values of variables x and y at node $k$. Hence, x and y are
%% not misreported as constants any more. The approach then generates the
%% prefix \vpath{ab(cdefgc)^3hijk}, which also brings values t=1,z=1 at node
%% $k$. The termination condition, which will describe in detail below, is
%% triggered at this point, and the approach stops with the constant result
%% t=1,z=1 at node $k$.

%\begin{figure}
%  \includegraphics[width=4in]{intra-system-rough.png}
%  \caption{VCFG of running example}
%  \label{fig:running-eg-vcfg}
%\end{figure}

\subsection{Assumptions}
\label{ssec:intra-assump}
Since the given abstract domain $\dlattice$ is assumed to be a complete
lattice, the set of all $\dlattice \rightarrow \dlattice$ transfer
functions also necessarily form a complete lattice, with the following
domination ordering: $f_1 \sqsubseteq f_2$ iff for all $d \in \dlattice$,
$f_1(d) \sqsubseteq f_2(d)$.
Backward DFAS makes a few additional assumptions on the lattice of transfer
functions. The first is that this lattice is of finite height. That is, all
strictly ascending chains of elements in this lattice are finite (although
no apriori bound on the sizes of these chains is required). This assumption
is required to ensure termination of our approach. The second is that a
representation of transfer functions is available, as are operators to
compose, join, and compare transfer functions. Thirdly, we need
distributivity, as defined below: 
for any $f_1, f_2, f \in \dlattice \rightarrow \dlattice$,
$(f_1 \sqcup f_2) \circ f = (f_1 \circ f) \sqcup (f_2 \circ f)$. The
distributivity assumption is required for soundness of the results, but is
required only if the given system contains procedure calls. 
%% We believe that it should be possible
%% to relax this assumption, but we leave this for future work. (The approach
%% also requires left distributivity of composition over join as well, but
%% this property follows simply from the definitions of function and join.)

Our final assumption is also required only in the presence of procedures.
It is that the procedures in $\funcs$ may send messages, but not have any
``receive'' statements. Only the main procedure is allowed to perform
receive actions from channels (it can send as well). Previous approaches
that address other sorts of data flow analysis or verification problems for
asynchronous systems with recursive procedures also have the same
restriction~\cite{sen2006model,jhala2007interprocedural,ganty2009verifying}.
This assumption is not as restrictive as it may seem.  For instance, in
\emph{event based systems}, which are a sub-class of general asynchronous
message passing systems, sending a message corresponds to generating an
``event'', while receiving a message corresponds to triggering an event
handler, which happens only at the outermost (dispatcher) level.  Event
based systems are deployed in varied  domains
such as UI-based applications, mobile applications, and reactive
server-side code.
%% Examples are UI-based web
%% applications using JavaScript, desktop and mobile applications that use
%% JavaAWT or JavaFX, systems like web servers, virtual networks, OS audit
%% systems, load balancers, and protocol implementations, which use libraries
%% like \emph{Node.js} and \emph{libevent}.

Our approach has no restriction that the given data lattice $\dlattice$ be
finite, and in this way it generalizes conceptually over previous data flow
analysis as well as verification approaches.
Examples of abstract domains that have been proposed in the literature that
are infinite and that satisfy all assumptions above are
LCP~\cite{sagiv1996precise} and ARA (Affine Relationships
Analysis)~\cite{muller2004precise}.  Our Forward DFAS approach
does not make the four assumptions listed above, but is not always
guaranteed to compute the precise JOFP (with or without procedure calls). 

%% 4. Define demand of a path.




%% If we assume for ease of discussion that there is a single channel in the
%% system, then for any message type $m$, $\demandpd{p}{d}[m]$ is intuitively
%% the minimum number of instances of message $m$ that need to be in the channel
%% \emph{before} $p$ executes in order for $d[m]$ instances of message $m$ to be
%% in the channel after $p$ executes.  We define $\demandp{p} =
%% \demandpd{p}{\zerovector}$, where $\zerovector$ is the vector of all zeroes.

%% A set of paths $C$ is said to \emph{cover} a path $p$ iff

%% \begin{itemize}
%% \item all paths in $C$ have the same start and end nodes
%%   (respectively) as $p$, and
%% \item the demand of each of these paths is less than
%%   or equal to $\demandp{p}$, and
%% \item 
%% the join of the path transfer functions of all these paths dominates the
%% path transfer function of $p$.
%% \end{itemize}


%% 5. Point to pseudo-code, and explain briefly the parameters, return value,
%%    and sPath.

\subsection{Backward DFAS algorithm -- intra-procedural component}
\label{ssec:intra-algo}


\begin{algorithm}
  \caption{Backward DFAS algorithm}
  \label{algo:intra}
  \begin{algorithmic}[1]
  \Procedure{ComputeJOFP}{$\targetnode$}
    
      \Comment{\begin{minipage}{4.8in}Returns JOFP
      from $\startnode \in \nodes$ to  $\targetnode
      \in \nodes$, treating $d_0 \in \dlattice$ as the entry value.\end{minipage}}

    \ForAll{$v \in \nodes$} \Comment{{\nodes} is the set of all nodes in the
VCFG}

      \State \sPaths{v} = $\emptyset$

    \EndFor

    \State
      For each intra-procedural VCFG edge $(v \vcfgtrans{f}{w}
      \targetnode$), add this edge to $\worklist$, $\sPaths{v}$.
      \label{step:intra:initw}

    \Repeat\label{step:intra:repeat}

      \State Remove any path $p$ from \worklist.\label{step:intra:removw}

      \State Let $v_1$ be the start node      of $p$.

      \ForAll{intra-procedural edges $e$ = $v_3 \vcfgtrans{f}{w} v_1$ in the
        VCFG}\label{step:intra:inner-loop-begin} 

        \If{\textsc{Covered}($e \concat p$) returns \fls}\label{step:intra:checkCov}

          \State Add the path ($e \concat p$) to \sPaths{v_3} and to
            \worklist. 
        
        \EndIf
      
      \EndFor\label{step:intra:inner-loop-end}

      \State \textsc{InterProcExt}($p$)\label{step:intra:callInter}

    \Until{{\worklist} is empty}\label{step:intra:until}

    \State $P \ = \ \{p \ \, | \, \ p \in \sPaths{\startnode},
      \demandp{p} = \zerovector\}$\label{step:intra:P}

    \State \textbf{return} $\bigjoin_{p \in P} \,
    (\ptf{p})(d_0)$\label{step:intra:return} 
      
  \EndProcedure

  \Procedure{Covered}{$p$}

    \Comment{\begin{minipage}{4.8in}Returns {\tru} iff there exist a set
        of paths in $\sPaths{v_1}$ that cover $p$, where $v_1$ is the
        start node of $p$. \end{minipage}}

    \State Let $v_1$ be the start node  of $p$.
    
    \State $C$ = $\{p' \ | \ p' \in \sPaths{v_1}, \demandp{p'} \leq
      \demandp{p} \}$\label{step:intra:covSet}

    \State \textbf{return} {$(\bigjoin_{p' \in C}\ptf{p'}) \dominates
      \ptf{p}$}\label{step:intra:ptfCov} 
    
  \EndProcedure
    
  \end{algorithmic}
\end{algorithm}

Our approach is summarized in
Algorithm~\ref{algo:intra}. \textsc{ComputeJOFP} is the main
routine. The algorithm works on a given iVCFG (which is an implicit
parameter to the algorithm), and is given  a $\targetnode$ node at which the
JOFP is to be computed.
A key data structure in the algorithm is {\sPathsName}; for any node
$v$, $\sPaths{v}$ is the set of all paths that start from $v$ and end at
$\targetnode$ that the algorithm has generated and retained so far.  The
{\worklist} at any point stores a subset of the paths in {\sPathsName}, and
these are the paths of the iVCFG that need to be extended backward.
The utility function \emph{demand} that is used in the algorithm is defined
as follows. \\[1em]
%% We now formalize the notion of \emph{demand} of
%% a path in the VCFG. We first introduce a function $\mu \equiv \lambda z \in
%% \mathbb{Z}.\ \mathit{max}(z,0)$.  $\mu$ also operates on vectors of
%% integers in the natural manner, that is, by application on each element.
%% For a path $p$, and vector $d \in {\natzero}^r$:
$
\begin{array}{lcll}
  \demandpd{p}{d} & = & \mathit{max}(d - w, \vec{0}),
      & \mathrm{if\ } p = (v \vcfgtrans{f}{w} z) \\
                & = & \mathit{max}(\demandpd{p'}{d} - w, \vec{0}), 
  & \mathrm{if\ } p = (e \concat p'),
  \mathrm{where\ } e \equiv (v   \vcfgtrans{f}{w} z) \\
  \demandp{p} & = & \demandpd{p}{\vec{0}} 
\end{array}
$\\

We now illustrate the steps of the algorithm (excluding its inter-procedural
component, for now)   using our running example
(Figure~\ref{fig:challenge}).  We use, for the purpose of illustration, 
\emph{Linear Constant Propagation} (LCP) as the given abstract domain
$\dlattice$.
In this analysis,
the transfer function of an edge (resp. path) maps the outgoing value of each
variable from the edge (resp. path) to \emph{either} a constant, \emph{or} to
a linear expression in the incoming value of at most one variable into the
edge (resp. path), \emph{or} to a special symbol $\top$ that indicates an
unknown outgoing value. Therefore, for instance, for the edge $g \rightarrow
c$ in our example, its transfer function can be represented symbolically as
t'=t,x'=x+1,y'=y,z'=z, where the primed versions represent outgoing values
and unprimed versions represent incoming values.
In the example, Node~$a$ is treated as $\startnode$, while
node~$k$ is $\targetnode$.


\begin{figure}
  \begin{tabular}{|l|l|l|c|c|l|}\hline
    & \parbox{0.7in}{Path from worklist} &
    \parbox{0.9in}{Extended path $p$} &
    \demandp{p} & \ptf{p} & \parbox{0.7in}{Covered by} \\\hline
    1 & & \vpath{hijk} & 3 & \id &  \\
    2 & \vpath{hijk} & \sout{\vpath{(hijk)^2}} & 6 & \id & \vpath{hijk} \\
    3 & \vpath{hijk} & \vpath{chijk} & 3 & \id & \\
    4 & \vpath{chijk} & \vpath{(cdefg)chijk} & 2 & t'=z,x'=x+1,y'=x,z'=1 & \\ 
    5 & \vpath{(cdefg)chijk} & \vpath{(cdefg)^2chijk} & 1 & t'=1,x'=x+2,y'=x+1,z'=1 & \\
    6 & \vpath{(cdefg)^2chijk} & \vpath{(cdefg)^3chijk} & 0 & t'=1,x'=x+3,y'=x+2,z'=1 & \\
    7 & \vpath{(cdefg)^3chijk} & \vpath{(cdefg)^4chijk} & 0 & t'=1,x'=x+4,y'=x+3,z'=1 & \\
    8 & \vpath{(cdefg)^4chijk} & \sout{\vpath{(cdefg)^5chijk}} & 0 & t'=1,x'=x+5,y'=x+4,z'=1 &
      \vpath{\{(cdefg)^3chijk}, \\
      & & & & & \ \vpath{(cdefg)^4chijk\}} \\\hline
    %% 9 & \vpath{chijk} & \vpath{abchijk} & 2 & t'=0,x'=0,y'=0,z'=0 & \\
    %% 10 & \vpath{cdefgchijk} & \vpath{abcdefgchijk} & 1 & t'=1,x'=1,y'=0,z'=1 & \\
    %% 11 & \vpath{(cdefg)^2chijk} & \vpath{ab(cdefg)^2chijk} & 0 & t'=1,x'=2,y'=1,z'=1 & \\
    %% 12 & \vpath{(cdefg)^3chijk} & \vpath{ab(cdefg)^3chijk} & 0 & t'=1,x'=3,y'=2,z'=1 & \\
    %% 13 & \vpath{(cdefg)^4chijk} & \sout{\vpath{ab(cdefg)^4chijk}} & 0
    %%   & t'=1,x'=4,y'=3,z'=1 & \vpath{\{ab(cdefg)^2chijk}, \\
    %%    & & & & & \ \vpath{ab(cdefg)^3chijk\}}\\\hline
  \end{tabular}
  \caption{Illustration of algorithm on running example}
  \label{fig:intra-illus}
\end{figure}

%% 5a. Then illustrate the approach using Fig. 9. Explain clearly, by invoking
%%    Lemmas 1 and 2, why covered paths can be dropped. Mention need to use
%%    path transfer functions -- data lattice alone does not suffice.

%%    In the end, explain why it is enough to consider zero-demand paths.


The illustration is tabulated in Figure~\ref{fig:intra-illus}.  In the
beginning, all edges incident onto {\targetnode} are generated and retained
(Line~\ref{step:intra:initw} in Algorithm~\ref{algo:intra}). That is, path
\vpath{jk} would be retained in $\sPaths{j}$. For the sake of brevity, in
Figure~\ref{fig:intra-illus}, from among the paths that are generated and
retained by the algorithm, we only show the ones that begin at nodes $h$ or
$c$.  Therefore, Row~1 in Figure~\ref{fig:intra-illus} shows the generation
of the path $\vpath{hijk}$, which would have been generated from
$\vpath{jk}$ after two more steps of growing in the backward
direction. Columns~3-5 in the figure show the new path $p$ that was just
generated and retained, its demand, and its path transfer function,
respectively. Since the number of counters is 1 in this example, the
demands are simply natural numbers rather than vectors.

%% In
%% Figure~\ref{fig:intra-illus}, see Row~1, where path $jk$ is generated and
%% stored (in $\sPaths{j}$. Each row in this figure indicates a step of the
%% algorithm (i.e., an iteration of the loop in
%% Lines~\ref{step:intra:repeat}-\ref{step:intra:until}).  The columns in
%% Figure~\ref{fig:intra-illus} have the following meanings:

%% \begin{itemize}
%% \item The third column (Extended path $p$) indicates the new path $p$ that
%%   is generated in this step.
%% \item The second column (Path from worklist) indicates the previously
%%   generated path that was pulled out of the worklist in this step and whose
%%   extension in the backward direction is the path $p$ that is
%%   produced in this step.
%% \item The meanings of fourth and fifth columns are self-explanatory. Note
%%   that we show the demands, which are vectors with a single element each in
%%   this case (corresponding to message $m$ in Figure~\ref{fig:challenge}),
%%   simply as numbers in the interest of brevity.
%%   We  will  touch upon the sixth column later.
%% \end{itemize}

The algorithm continually picks up a path from the worklist
(Line~\ref{step:intra:removw}), and extends this path in the backward
direction in all possible ways by a single edge
(Lines~\ref{step:intra:inner-loop-begin}-\ref{step:intra:inner-loop-end}). After
four steps of extension in this way, the path \vpath{hijk} would result in
the new path \vpath{hijkhijk}, which we abbreviate as \vpath{(hijk)^2}. This
new path is depicted in Row~2 in Figure~\ref{fig:intra-illus}. Column~2 in
this row indicates that the new path was obtained by extending the previously
generated path
\vpath{hijk}. 

\paragraph{The covering check}

However, the path $\vpath{(hijk)^2}$ is not retained in $\sPaths{h}$, and
its further backward extensions (i.e., paths that end with the form
\vpath{(hijk)^i}, $i \geq 2$) are not produced at all. This step is key to
ensuring termination of the algorithm, as otherwise cycles in the VCFG would be
unrolled indefinitely.  A set of paths $C$ that are already retained
are said to \emph{cover} a newly generated path $p$ if each path in $C$ has
the same two terminal nodes as $p$ and has demand equal to or less than $p$,
and the join of the path transfer functions of the paths in $C$ dominate 
$\ptf{p}$.  This check is accomplished by routine~\textsc{Covered}, which is
called from Line~\ref{step:intra:checkCov}. Covered paths are not retained in
$\sPathsName$ and do not go into the worklist, either. Thus, in Row~2 of
Figure~\ref{fig:intra-illus}, the path \vpath{(hihk)^2} is shown
crossed out, and Column~6 indicates that \vpath{hijk} is the covering path.


%% %% However,
%% %% in the interest of brevity of illustration, we will view the algorithm here
%% %% as extending each path in a single step by a sequence of edges. Row~2 in
%% %% Figure~\ref{fig:intra-illus} shows an extension of path $jk$, namely, path
%% %% $chijk$, which is stored in $\sPaths{c}$.

%% \subsubsection{The role of the covering check}
%% \label{sssec:covCheck}

%% In the algorithm, a path newly generated in any step is \emph{not} stored
%% in $\sPathsName$ (i.e., is thrown away) if a set of previously generated
%% and stored paths between the same start and end nodes \emph{cover} this
%% path. The notion of covering was defined earlier in
%% Section~\ref{ssec:intra-assump}. The covering check forms the core idea
%% behind the algorithm that ensures termination and soundness.

%% In Algorithm~\ref{algo:intra} the covering condition is checked by
%% Procedure~\textsc{Covered}, which is called from 
%% Line~\ref{step:intra:checkCov} in the main procedure.

%% The following two lemmas, and their corollary, characterize why covered
%% paths can be dropped.

%% \textbf{Lemma 1}. If $p_1$ and $p_2$ are both paths from a node $v_i$ to a
%% node $v_j$ such that $\demandp{p_1} \leq \demandp{p_2}$, and if $p_0$ is
%% any path ending at $v_i$, then $\demandp{p_0 \concat p_1} \leq
%% \demandp{p_0 \concat p_2}$.

%% \textbf{Lemma 2}. If $p_1$ is a path from a node $v_i$ to a node $v_j$, and
%% $P_2$ is a set of paths from $v_i$ to $v_j$ such that $(\bigjoin_{p_2 \in P_2}
%% \ptf{p_2}) \dominates \ptf{p_1}$, and if $p_0$ is any path ending at $v_i$,
%% then $(\bigjoin_{p_2 \in P_2} \ptf{p_0 \concat p_2}) \dominates \ptf{p_0 \concat p_1}$.\\

%% The lemmas above are easy to prove, as they follow directly from the
%% definitions of ``demand'' and ``join''.

The following lemma characterizes why it is sound  to throw away a
covered path. 

\textbf{Lemma 1.}  If two paths $p_2$ and $p_3$ cover a path $p_1$ (can
be generalized to any finite set of paths covering $p_1$), and if all these
three paths are from a node $v_i$ to a node $v_j$, and if $p_0$ is any path
ending at $v_i$ such that $p_0 \concat p_1$ is a feasible path, then:

\begin{itemize}
\item $p_0 \concat p_2$ and $p_0 \concat p_3$, both are feasible paths
  
\item for any data value $d_i \in \dlattice$, $(\ptf{p_0 \concat p_2}(d_i)
  \join \ptf{p_0 \concat p_3}(d_i)) \dominates \ptf{p_0 \concat
    p_1}(d_i)$.  \hfill$\Box$
\end{itemize}

%% The second property above is easy to see, as it follows from the definition
%% of function composition and join. The first property above is not so
%% obvious; it follows from Lemma~1, and from the fact that a path $p$ in the
%% VCFG is feasible iff $\demandp{p} = \zerovector$.

It follows from the lemma above that $p_1$ can be dropped if $p_2$ and
$p_3$ are retained, because  any backward extension of
$p_1$ that is feasible and hence normally ought to be considered in
order to produce a sound data value at node $v_j$, such as $p_0 \concat
p_1$, is itself covered by the corresponding extensions of $p_2$ and $p_3$,
i.e., by $p_0 \concat p_2$ and $p_0 \concat p_3$. Since $p_2$ and $p_3$
have been retained by the algorithm, all their backward extensions will be
generated, and hence soundness is assured.

%% Note, our algorithm needs to work with transfer function representations of
%% paths, because when we grow paths in the backward direction and check
%% whether a set of paths cover a path, we do not know apriori all possible
%% data values (from lattice $\dlattice$) that can flow into the start nodes
%% of these paths; we only know the start value $d_0$ at $\startnode$.

\paragraph{Continuing the illustration of the algorithm}

Rows~3-7 in Figure~\ref{fig:intra-illus} depict backward extensions of the
path \vpath{hijk} that get generated and retained. These paths correspond to
unrolling the first cycle in Figure~\ref{fig:challenge} upto four times. The
path \vpath{(cdefg)^5 hijk} (Row~8) is covered by the paths in Rows~6 and~7,
and is hence thrown away. Note that the join of the path transfer functions
of the paths in Rows~6 and~7 works out to (t' = 1, x' = $\top$, y' = $\top$,
z' = 1), and this dominates the path transfer function of the path in
Row~8. Effectively, this means that for any data value $d$ that happens to arise
at node $c$, if $d$ transferred via the path \vpath{(cdefg)^5 hijk} results
in a value $d'$ at node $k$, then if the same $d$ is transferred via the two
paths in Rows~6 and~7 and the results are joined at node $k$, this joined
value is guaranteed to dominate $d'$. This, in conjunction with the fact that
the paths in Rows~6 and~7 have demand less than or equal to the path in
Row~8, guarantees that it is sound to throw away the path in Row~8 (see
Lemma~1). Also, since \vpath{(cdefg)^5 hijk} is thrown away, its backward
extensions that would iterate the first cycle 6 or more times, would not
be generated at all.

Finally, when the paths in Rows~5-7 get extended back to node $a$ by
prepending the prefix \vpath{ab}, the resulting paths are zero-demand
  paths. The final result returned by the algorithm (see
  Lines~\ref{step:intra:P} and~\ref{step:intra:return} in
  Algorithm~\ref{algo:intra}) is the join of the values transferred by these
  zero-demand paths starting from the given entry value $d_0 \in \dlattice$.

Effectively, in this example, the algorithm first discovered that one
iteration of the second cycle suffices. Then, using the demand of this one
iteration, the algorithm  discovered that up to four
iterations of the first cycle suffice to produce a sound (and precise) final
JOFP result at node $k$.

%% Row~3 in Figure~\ref{fig:intra-illus} depicts the generation of an
%% extension of path $jk$, namely, $jkhijk$. This extension corresponds to a
%% full iteration of the second cycle in Figure~\ref{fig:challenge}.  Path
%% $jk$ itself covers path $jkhijk$. Both these paths have demand zero, and
%% both have $\id$ as path transfer function. The strikeout in Row~3 indicates
%% that path $jkhijk$ is thrown away (not stored).

%% Rows~4-7 indicate three further backward extensions of path $jk$,
%% corresponding to one, two, three, and four iterations, respectively, of the
%% first cycle in Figure~\ref{fig:challenge}. These paths are not
%% discarded. For instance, the path in Row~7 is not discarded because there
%% is only path that has lower demand than this path (the path in Row~6), and
%% transfer function of the path generated in Row~6 (shown in the fifth
%% column) does not dominate the transfer function of the path generated in
%% Row~7.

%% The fact that all these paths are stored is the reason why the eventual
%% result at node~$k$ turns out sound. Our backward traversal approach, in
%% conjunction with demands, ensures that all these paths are generated. The
%% path $chijk$, generated in Row~2, has a demand of 3; in order to satisfy
%% this demand, up to four iterations of cycle are generated (Rows~4-7). If
%% fewer iterations of this cycle had been enumerated, say only up to two
%% iterations, then too few feasible paths would have reached node~$k$. In
%% particular, only the path  that goes through two iterations of the first
%% cycle would have reached node~$k$. This would have resulted in unsoundness
%% (i.e., in all four variables being reported as constants). 

%% The path generated in Row~8, corresponding to five iterations of
%% the first cycle, is discarded. As a result,  higher iteration counts of the
%% first cycle are not generated at all. The path in Row~8 is covered by the
%% paths in Rows~6 and~7. Hence, termination is assured.

%% Rows~9-10 correspond to backward extensions of the paths in Rows~2-7 all
%% the way up to the start node~$a$. Of these paths, the ones in Rows~11
%% and~12 have demand of zero. Recall, a demand of zero indicates a feasible
%% path. The initial data value $d_0$ (which is, say, $\top$) is sent through
%% these two paths up to node~$k$ (see
%% Lines~\ref{step:intra:P}-\ref{step:intra:return} in
%% Algorithm~\ref{algo:intra}). These paths both bring a value of 1 for
%% variables t and z, and non-agreeing values for x and y (thus resulting in
%% them reported as non-constant, which is the sound result). 



==> vcfg-construction-rules.tex <==
\begin{figure}
\centering
\begin{tabular}{c}
\begin{math}
\process_i \in \asystem, \hspace{10pt} \process_i =(Q_i, q_{i0}, V_i, A_i, C_i, M_i, \delta_{\process_i}) \hspace{10pt} \langle q_{i1}, \send{c}{m}, q_{i2}\rangle \in \delta_{\process_i} 
\end{math}\\
\begin{math}
 a = \id \hspace{10pt} w = w_0[\counterIndex{\mathrm{c}}{\mathrm{m}} \mapsto 1]  
\end{math}\rule[-0.25em]{0in}{0in}\\ \hline
\rule[1.5em]{0in}{0in}
\begin{math}
 \langle q_{11}, \ldots, q_{i1}, \ldots, q_{n1}\rangle  \vcfgtrans{a}{w}   \langle q_{11},  \ldots, q_{i2}, \ldots, q_{n1}\rangle
\end{math}
\rule[-0.25em]{0in}{0in}
\end{tabular}
~~$[\texttt{t-send}]$

\vspace{15pt}
\centering
\begin{tabular}{c}
\begin{math}
\process_i \in \asystem, \hspace{10pt} \process_i =(Q_i, q_{i0}, V_i, A_i, C_i, M_i, \delta_{\process_i}), \hspace{10pt}  \langle q_{i1}, \recv{c}{m}, q_{i2}\rangle \in \delta_{\process_i} 
\end{math}\\
\begin{math}
 a = \textit{id} \hspace{10pt}  w = w_0[\counterIndex{\mathrm{c}}{\mathrm{m}} \mapsto -1]  
\end{math}\rule[-0.25em]{0in}{0in}\\ \hline
\rule[1.5em]{0in}{0in}
\begin{math}
\langle q_{11}, \ldots, q_{i1}, \ldots, q_{n1}\rangle  \vcfgtrans{a}{w}   \langle q_{11}, \ldots, q_{i2}, \ldots, q_{n1}\rangle
\end{math}
\rule[-0.25em]{0in}{0in}
\end{tabular}
~~$[\texttt{t-receive}]$

\vspace{15pt}

\centering
\begin{tabular}{c}
\begin{math}
\process_i \in \asystem, \hspace{10pt} \process_i =(Q_i, q_{i0}, V_i, A_i, C_i, M_i, \delta_{\process_i}), \hspace{10pt}  \langle q_{i1}, \alpha, q_{i2}\rangle \in \delta_{\process_i}
\end{math}\\
\begin{math}
 a = \lambda \textit{val} \in (V \rightarrow \mathbb{Z}).\left( \lambda v \in V.\left( \begin{cases} (\alpha(\textit{val}))(v) \hspace{3pt} \textit{ if }\, v \in V_i \\ \textit{val}(v) \hspace{3pt} \textit{otherwise} \end{cases} \right) \right) \hspace{10pt} 
\end{math}\rule[-0.25em]{0in}{0in}\\ \hline
\rule[1.5em]{0in}{0in}
\begin{math}
\langle q_{11}, \ldots, q_{i1}, \ldots, q_{n1}\rangle  \vcfgtrans{a}{w_0}   \langle q_{11}, \ldots, q_{i2}, \ldots, q_{n1}\rangle
\end{math}
\rule[-0.25em]{0in}{0in}
\end{tabular}
~~$[\texttt{t-action}]$

\caption{Edges and label functions construction rules for $\asystem$ and $\vcfggraph$}
\label{fig:vcfgConsRules}
\end{figure}

